Fair Conformal Classification via Learning Representation-Based Groups

Conformal prediction methods provide statistically rigorous marginal coverage guarantees for machine learning models, but such guarantees fail to account for algorithmic biases, thereby undermining fairness and trust. This paper introduces a fair conformal inference framework for classification tasks. The proposed method constructs prediction sets that guarantee conditional coverage on adaptively identified subgroups, which can be implicitly defined through nonlinear feature combinations. By balancing effectiveness and efficiency in producing compact, informative prediction sets and ensuring adaptive equalized coverage across unfairly treated subgroups, our approach paves a practical pathway toward trustworthy machine learning. Extensive experiments on both synthetic and real-world datasets demonstrate the effectiveness of the framework.

==> bin.tex <==
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motivation of our work}\label{Sec:motivation}
\tl{to decide which goes to intro, which stays here}

 we can describe the 
each sample group $\mathcal{G}$ is defined as 
we consider a set-valued random variable $\mathcal{G}_\mathbf{H}$ parameterized by the random vector $\mathbf{H} = [H_1, \dots, H_N]$ each component of which is a random indicator variable. % s $\{H_i\}_{i=1}^N$, i.e.,
For a realization of $\mathbf{h}=[h_1, \cdots, h_n]$ of $\mathbf{H}$, 
%
\begin{equation}\label{Eq:group}
\mathcal{G}_\mathbf{h} := \{ X_i : i \in [N], h_i = 1 \},
\end{equation}
$\mathbf{H} = [H_1, \dots, H_N]$ satisfies that its components are independent of each other under the condition of all given features $\{X_i\}_{i=1}^N$. 

Let  $\mathcal{X}=\{X_1, \cdots, X_N\}$ be the set of all features. \tl{I am actually quite confused here, $X_i$ is normally used for the calibration set.}

\hide{
We consider a set-valued random variable $\mathcal{G}_{[S_1, \cdots, S_N]}$ where $S_i$'s are $\{0,1\}$-valued i.i.d. random variables. We have $X_i\in \mathcal{G}_{[S_1, \cdots, S_N]}$ iff $S_i=1$ for each $i\in [N]$. 

$S_i\mid Z_i$ is governed by a Bernoulli distribution where $Z_i=f(X_i)$, where $f$ denotes ... 

\[
\mathbb{P}[Y_{N+1} \in \hat{C}(X_{N+1}) \mid H_{N+1}=1] \geq 1 - \alpha
\]

We consider a set-valued random variable $\mathcal{G}_\mathbf{H}$ parameterized by the random vector $\mathbf{H} = [H_1, \dots, H_N]$ where $H_i$'s are iid, each of which is governed by a Bernoulli distribution. 
% %For a realization of $\mathbf{h}=[h_1, \cdots, h_n]$ of $\mathbf{H}$, 
% %
$\mathcal{G}_\mathbf{H}= X\subseteq \mathcal{X}$ such that $X_i\in \mathcal{G}_\mathbf{H}$ iff $H_i=1$ for all $i\in [N]$. 
}
\tl{I am not sure this is what we want. Basically, for X1,... XN, we first get Z1, ..., ZN, then we can sample a 0-1 vector to form $\mathcal{G}$ which is a set. But the event that $ X_{N+1}\in \mathcal{G}_{[S_1,\cdots, S_N]}$ looks very weird, and is not quite consistent with th previous work.}

\tl{I actually suspect here $X_i$'s do not refer to calibration set, but refer to attributes.}
 
The distribution of $\mathcal{G}_\mathbf{H}$ conditioned on $X_i$'s is given by 

\begin{equation}\label{Eq:H}
\mathbf{H} \mid \{X_i\}_{i=1}^N \sim \prod_{i=1}^N \operatorname{Bernoulli}(\mathbf{P}(S_i=1 \mid Z_i)),
\end{equation}

However, various groups $\mathcal{G}$ usually suffer from different degrees of algorithmic bias, and the groups that need to be protected (characterized by the poor conditional coverage) are typically unknown in real-world applications. \tl{examples?}

To solve this concern, existing work AFCP~\citep{zhou2024conformal} proposes 
% employ a linear decision stump 
to mine the groups that are discriminated against via the feature selection using a linear decision stump.  
% \tl{what is the formal meaning of this linear decision stump?}.
Specifically, for a test point $X_{N+1}$, they compute a conditional miscoverage score for each single \emph{discrete} feature of $X_{N+1}$ and pick the top-$k$ features with the highest scores as the selected features, where $k$ is a hyperparameter which decides the number of selected features. 
Arbitrary $X\in \mathcal{X}$ with the same value on the selected features as $X_{N+1}$ is assigned to the group $\mathcal{G}$ \tl{I do not quite understand this (unfinished?) senstence}

\tl{check this please}
Suppose there are two features: a continuous feature \textit{Age}
% \textit{Age $:=\{$Underage: 0, Adult: 1$\}$} 
and a discrete feature \textit{Gender $:=\{$Male, Female$\}$}, and $X_{N+1}$ is an instance of Male of age 50. Then one group (for Age) includes all samples with an age 50, and another group (for Gender) includes all samples who are Male. AFCP computes conditional miscoverage scores for these two groups. 




% For a decision-making process driven by machine learning (e.g., medical diagnostics, job screening and recidivism prediction) %, loan approval, fraud detection), 
% it is essential for the predictions to be accompanied by a level of confidence to quantify uncertainty~\cite{vovk2005algorithmic,smith2024uncertainty}.
% Conformal prediction (CP) is a promising uncertainty quantification method, providing statistically rigorous uncertainty sets for black-box machine learning models~\cite{babbar2022utility,straitouri2023improving,straitouri2023designing,cresswell2024conformal}. 
% %Conformal prediction (CP) is a machine learning framework for uncertainty quantification used in decision-making processes (e.g., loan approval, fraud detection)~\cite{vovk2005algorithmic,smith2024uncertainty}.  
% In standard classification, for any test input $x$, the posterior distribution $\tilde{\pi}_y(x)= P(Y=y\mid X=x)$ on classes $[K]:=\{1, \cdots, K\}$ is calculated. %This does not guarantee safe deployment. 
% Conformal prediction leverages an additional
% calibration step to guarantee a user-specified (marginal) coverage: by producing a prediction set $\mathcal{C}(x)\subseteq [K]$, it guarantees the true class of $x$ is included in $\mathcal{C}(x)$ with a user-chosen probability, % $1-\alpha$, 
% when the calibration samples are exchangeable with the test samples. 


%%%%%%%%%%%%%%%%%%%% this is just for later use %%%%%%%%%%%%%%%%
In conformal prediction, it is important to distinguish between marginal and conditional coverage guarantees. Marginal coverage ensures that, averaged over the entire data distribution, the prediction set contains the true label with probability at least 
$1-\alpha$. Formally,
$ P(Y\in \hat{C}(X))\geq 1-\alpha$,
where the probability is taken over both inputs and outputs. This guarantee is relatively easy to achieve and is what standard conformal methods provide.

By contrast, conditional coverage requires the guarantee to hold for each input (or subgroup of inputs), i.e.,
$\forall x$, $P(Y\in \hat{C}(X)\mid X=x)\geq 1-\alpha$.
This is a much stronger notion of validity, as it demands correct coverage across all regions of the feature space, not just on average. However, achieving conditional coverage is generally infeasible in finite-sample settings without making strong distributional assumptions, and attempts to enforce it often lead to excessively conservative prediction sets.

%%%%%%%%%%%%%%%%%%%%%%%%
% intuition of adaptability
% A key design consideration for conformal prediction is adaptivity: we want the procedure to return larger sets for harder inputs and smaller sets for easier inputs. 

% It is important to keep in mind that the CP procedure with the smallest average set size is not necessarily the best. A good CP procedure will give small sets on easy inputs and large sets on hard inputs in a way that faithfully reflects the model's uncertainty. This adaptavity is not implied by the marginal coverage, but it is non-negotiable in practical deployments of conformal prediction. 

% % Precise metrics for adaptivity that allow users to check a conformal procedure and to compare multiple alternative conformal procedures. 
% Adaptivity is typically formalized by the conditional coverage. That is, for each value of the input $X_{\rm test}$, we seek to return prediction sets with $1-\alpha$ coverage. This is a stronger property than the marginal coverage that CP is guaranteed to achieve. Indeed, in the most general case, conditional coverage is impossible to achieve \cite{Vovk12}, i.e., conformal procedures are not guaranteed to satisfy conditional coverage. It is imperative to check how close a CP comes to approximate it. (feature-stratified coverage metric, size-stratified coverage metric)



\textbf{Group-balanced conformal prediction}: want prediction intervals that have equal error rates across certain subsets of the data. 

Class-conditional CP

\tl{copied from Romano's paper.}
We propose a concrete procedure, which acts as a wrapper around the predictive model, to produce
perfectly valid prediction intervals that provably satisfy the equalized coverage constraint for any black box algorithm, sample size and distribution. Such a procedure can be formulated by refining tools from conformal inference, a general methodology for constructing prediction intervals [18–24]. Our contribution is nevertheless a little outside of classical conformal inference as we seek a form of conditional rather than marginal coverage guarantee [25–27].

\tl{to be adapted}
Conformal inference with \emph{equalized coverage}~\cite{romano2020malice} 
an appealing approach.

Equalized coverage aims to ensure that the prediction sets attain their coverage not only on average for the whole population (e.g., above 90\%) but also at the same level within each group of interest. While this does not necessarily imply that the prediction sets will have equal size on average across different groups, 
%—since it is possible the predictive model may be more or less accurate for different groups—
it objectively communicates the possible limitations of a model. This transparency helps decision makers recognize when predictions may be less reliable for specific subgroups, allowing them to either avoid unnecessary actions or adopt more cautious strategies in cases of higher uncertainty, thereby minimizing the potential harm from inaccurate predictions.

A limitation of %the method developed in [17] for conformal inference with 
equalized coverage is that it does not scale well to situations involving diverse populations with multiple sensitive attributes. In such cases, it necessitates splitting the data into exponentially many subsets, significantly reducing the effective sample size and leading to less informative predictions. 

Balancing this trade-off between efficiency (i.e., %aiming for 
highly informative predictions with small set sizes) and fairness (i.e.,
ensuring unbiased treatment) is challenging. % and requires novel approaches. This paper introduces
% a method to address this by providing equalized coverage conditional on carefully chosen features,
% informed by the model and data. 

While it cannot guarantee equalized coverage for all sensitive groups, it seeks a reasonable compromise with finite data sets, mitigating significant biases while
retaining predictive power.

\tl{to be adapted. This is just a placeholder}
% When multiple sensitive attributes are involved, the concept of equalized coverage is extended to \emph{exhaustive equalized coverage} \citep{zhou2024conformal}. However, a downside of this approach is that the calibration subsets may be too small if $M$ is large, leading to uninformative predictions for even moderate values of K. This limitation forms the starting point of our work. \tl{to be rephrased, basically a statistical barrier}

% \emph{Adaptively Fair Conformal Prediction.} In practice, for a given model and data set, different groups may not exhibit the same need for rigorous equalized coverage guarantees, as conformal predictions may be able to approximately achieve the desired coverage even without explicit constraints. Algorithmic bias typically affects only a minority of the population, so standard prediction sets with marginal coverage may approximately satisfy the marginal coverage for most groups. Adaptively Fair Conformal Prediction (AFCP) %, a new method that efficiently identifies and addresses groups suffering from algorithmic bias 
% was proposed in a data-driven
% way, adjusting their prediction sets to equalize coverage without sacrificing informativeness.

==> iclr2026-3/010_introduction.tex <==
%\subsection{uncertainty quantification and algorithmic fairness}
The rapid advancement of modern machine learning models, especially deep neural networks, has enabled their deployment in high-stake decision-making situations such as medical diagnoses~\citep{kaur2020medical}, resume filtering~\citep{deshpande2020mitigating}, and financial fraud detection~\citep{kamuangu2024review}. Despite their strong average performance, real-world deployment raises critical challenges, notably in uncertainty quantification~\citep{guo2017calibration,ahmed2023deep} and algorithmic fairness~\citep{berk2024improving,almasoud2025algorithmic}.

Ensuring reliable decision-making necessitates the development of unbiased uncertainty measures, as even highly accurate models are prone to producing over-confident and erroneous predictions~\citep{ovadia2019can}.
%To ensure reliable decision-making, as even highly accurate models could produce overconfident and erroneous predictions~\citep{ovadia2019can}, %underscoring the need for 
%unbiased uncertainty measures. 
Conformal Prediction (CP,~\citep{vovk2005algorithmic,smith2024uncertainty}) has emerged as a key framework for providing distribution-free, model-agnostic prediction sets with user-specified (marginal) coverage guarantees. These sets provide reliable uncertainty information for decision-makers especially when the set size is small (i.e., with high efficiency).
% However, marginal coverage alone is insufficient to ensure conditional coverage—i.e., consistency in prediction reliability across different subgroups.\xsr{revise}

On the other hand, algorithmic biases often manifest as disproportionately poor performance on the subgroup defined by specific feature conditions (e.g., \textit{Race=Black \& Gender=Female}), which may arise from imbalanced data distribution or model inherent limitations~\citep{hellman2020measuring}. These biases underscore the need for algorithmic fairness mechanisms that extend beyond average performance to ensure equitable treatment across all groups~\citep{fabris2022algorithmic,das2023algorithmic}. 
However, there may exist tensions between the efficiency of CP and algorithmic fairness, because the former desires a small prediction set, while the latter %encourages the set size 
may necessitate %to increase for acquiring 
larger sets for equal conditional coverage across all subgroups~\citep{gibbs2025conformal}.


%To tackle the efficiency–fairness trade-off, 
Conformal prediction with \emph{equalized coverage}~\citep{romano2020malice} provides a pragmatic approach to the efficiency–fairness trade-off. This approach ensures that the target coverage level (e.g., 90\%) is satisfied not only marginally over the entire population, but also conditionally on each protected group of interest. 
%It does not require prediction sets to be of equal size across different groups, as model accuracy may vary therein. Instead, it provides a more objective indication of model limitations.
%Such transparency enables decision-makers to recognize less unreliable predictions and adopt more cautious strategies, thereby mitigating risks associated with algorithmic bias.
However, acquiring prediction sets with equalized coverage is challenging,
as the number of all plausible groups of interest is exponential in the number of features.
A straightforward enumeration is practically infeasible both statistically and computationally, %significantly reduces the effective sample size for each group and is a heavy burden for time efficiency, 
especially on multi-dimensional (continuous) features.
Indeed, \citet{romano2020malice} only takes each single feature as the condition of groups (e.g., a group defined by $\textit{Gender=Female}$), which is an arguably insufficient %approximation to 
representation of the entire space of groups.


% Group-balanced conformal prediction is a refinement of conformal prediction (CP) motivated by fairness concerns. To navigate this efficiency-fairness trade-off, conformal prediction with \emph{Equalized Coverage}~\citep{romano2020malice} provides an attractive compromise solution.
% The goal of equalized coverage is to guarantee that the target marginal coverage rate (e.g., 90\%) is met not just across the entire population, but also for all protected groups of interest.
% While this does not necessarily imply that the prediction sets will have equal size on average across different groups—since it is possible the predictive model may be more or less accurate for different groups—it objectively communicates the possible limitations of a model.
% This transparency allows decision-makers to identify unreliable predictions and adopt more cautious strategies, thereby reducing potential risks from algorithmic biases.

% Equalized coverage guarantees that prediction sets meet the target coverage rate both overall and within every subgroup, reflecting potential variations in model accuracy through differing set sizes. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Achieving equalized coverage}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/intro.pdf}
    \vskip -0.5em
    \caption{An illustrative example. The group space is divided into four parts by the feature {\em Race} and {\em Gender}. Hard samples (red triangles) are unfairly treated by the classifier, and easy samples (green circles) are normally treated. Note that a single feature (either Race or Gender) cannot discover the unfair subgroups (both have four triangles and four circles). Stronger expressiveness is desirable to capture the unfair subgroup ``\textit{White Female} or \textit{Black Male}''.}
    % \vskip -1.0em
    \label{F:intro}
\end{figure}

%\tl{data-driven equalized coverage}
%Nevertheless, it is challenging to 

Later, \citet{zhou2024conformal} observe that 
%that rigorous equalized coverage is often group-specific: while standard marginal prediction sets typically suffice for the majority of the population, 
algorithmic biases often concentrate on a minority of subgroups, %given a model and an observed dataset. 
%To address this issue,
%Based on this observation,
%\citet{zhou2024conformal} 
and propose adaptively fair conformal prediction (AFCP) %adaptive equalized coverage 
to identify these potentially disadvantaged subgroups. %subgroups that may suffer from algorithmic biases.
In a nutshell, AFCP computes the conditional coverage score for each discrete feature and selects the top-$k$ sensitive features with a greedy strategy (where $k$ is a hyperparameter). 
%
However, this group identification method still has limited expressiveness. For example, it cannot capture 
groups defined by a nonlinear combination of features, such as Exclusive OR (see the subgroup ``\textit{White Female} or \textit{Black Male}'' %derived from XOR  %is a \emph{linear inseparable} group, which is 
%lies beyond AFCP, as shown 
in Fig.~\ref{F:intro}).
Additionally, AFCP is based on Na\"{i}ve Bayes, which incurs a high computational cost and restricts its applicability to continuous features.
% Generally speaking, previous work saves the data resource and computation cost by sacrificing the expressiveness for some specific groups defined by high-level feature representations. 
 
% A limitation of %the method developed in [17] for conformal inference with 
% equalized coverage is that it does not scale well to situations involving diverse populations with multiple sensitive attributes. In such cases, it necessitates splitting the data into exponentially many subsets, significantly reducing the effective sample size and leading to less informative predictions. 

\subsection{Our Contributions}
In this paper, we propose a new group-fair conformal prediction method, \textbf{fair conformal prediction for representation-based groups} (\name), which accommodates both group expressiveness and time efficiency.
Different from existing work~\citep{romano2020malice,zhou2024conformal} which directly extracts groups from the raw input feature $X$, our approach encodes $X$ into a %n intermediate 
latent representation $Z$ via a mapping $Z=f(X)$, and learns unfair groups characterized by the low group coverage %\tl{not quite clear about unfair group}  
based on $Z$.
The introduction of %the latent representation 
$Z$ as a high-level representation of features strengthens the expressiveness of models,  %capture more possible 
allowing a thorough exploration of groups.  
Meanwhile, we can enhance the interpretability by reconstructing input $X$ from the encoding $Z$. %\tl{(2) is a bit weak, it is a remedy not a benefit}
To this end, we carefully design an encoder-decoder architecture and the optimization objective, based on the principle of variational inference.

In addition, we propose a \emph{nonlinear} version of the conditional coverage metric WSC~\citep{cauchois2021knowing}, namely $\text{WSC}^+$, aiming to evaluate the conditional coverage of unfairly treated groups more precisely. This allows users to check a conformal procedure and to compare multiple alternative conformal procedures. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The main contributions of this paper are summarized as follows. 
First, we propose a new conformal prediction method %\name, 
to enhance the expressiveness of unfair group identification.
Second, we extend the traditional conditional coverage metric WSC to a nonlinear version $\text{WSC}^+$ for more accurate evaluation.
Comprehensive experiments on both synthetic and real-world datasets confirm the effectiveness and efficiency of our proposed method.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \emph{Structure.} 
% Section~\ref{sec:prel} briefly introduces conformal prediction.
% %Section~\ref{sec:moti} gives the theoretical results on the efficiency-entropy trade-off. 
% Section~\ref{sec:method} presents the proposed methods and Section~\ref{sec:exp} shows the experimental results. Section~\ref{sec:rel} discusses the related work, and Section~\ref{sec:con} concludes the paper.






==> iclr2026-3/020_preliminary.tex <==


% \textbf{Notations.} 
% %\tl{we may unify capital/lower case for x and y.}
% We focus on multiclass classification (with $K$ classes). 
% Assume $D=\{(X_i, Y_i)\}_{i=1}^{n+1}$ of i.i.d. (or simply exchangeable) observations sampled from an (unknown) 
% %the 
% testing 
% distribution $P_{XY}$.   
% We denote the (oracle) conditional distribution $P_{Y \mid X}$ %of $Y$ given $X$ 
% by $\pi_y(x) = P(Y=y \mid X = x)$. 
% Furthermore, a black-box base classifier undergoes %pre-training and 
% adapting to %approximate the oracle distribution, with its 
% prescribe prediction %represented as 
% $\hat{\pi}_y(x)$.

% \textbf{CP Framework.} 
% %Conformal prediction aims to establish a formal guarantee for the model prediction via uncertainty quantification.
% % Considering the efficient computation, we focus on the split conformal prediction method for distribution-free prediction~\cite{vovk2005algorithmic}.
% % Let $\mathcal{D}=\{(x,y)\}_{x,y\in \mathcal{X}\times \mathcal{Y}}$ be an overall dataset and CP splits the dataset $\mathcal{D}$ into four subsets, including training set $\mathcal{D}_{train}$, validation set $\mathcal{D}_{valid}$,  calibration set $\mathcal{D}_{calib}$ and test set $\mathcal{D}_{test}$. 
% % we withhold a fraction of data as the calibration set $\mathcal{D}_{calib}$ in order to conduct conformal prediction later on.
% % Given an overall dataset $D$, 
% % unlike the standard training-validation data split~\citep{xxx}, 
% % If the assumption of data exchangeability between $\mathcal{D}_{calib}$ and $\mathcal{D}_{test}$ is satisfied, i.e., $\mathcal{D}_{calib}\cup (X_{n+1},Y_{n+1})$ is exchangeable, 
% Given $D_{\mathrm{cal}} =\{(X_i, Y_i)\}_{i=1}^{n}$ as the calibration set and 
% %It often requires a held-out calibration set %held back 
% %to gauge the threshold of a so-called non-conformity score. 
% %Typically, 
% a user-defined miscoverage rate  $\alpha \in (0,1)$,
% CP typically proceeds in the following three steps:

% \textit{(1) Non-conformity score definition.} CP first heuristically defines a non-conformity score function $V(x, y)$, which indicates how the class $y$ conforms to the predictive result $\hat{\pi}(x) = [\hat{\pi}_1(x), \dots, \hat{\pi}_K(x)]$. 
% For example, the non-conformity score $V(x,y)$ can be defined as the sum of the probabilities of all $K$ classes in $\hat{\pi}(x)$ except class $y$.

% \textit{(2) Uncertainty calibration.} 
% CP then evaluates the non-conformity score for each data point $(X_i, Y_i)\in D_{\mathrm{cal}} $, resulting in the non-conformity score set $\{V(X_i,Y_i)\}_{i=1}^n$.  
% Subsequently, it sets a threshold $\hat{\eta}$ as its $(1-\alpha)(1+1/n)$-quantile. 
% %of %the non-conformity score set  $\{V(X_i,Y_i)\}_{i=1}^n$.

% \textit{(3) Prediction set construction.} For a new sample $X_{n+1}$, conformal prediction computes the corresponding prediction set by $\mathcal{C}(X_{n+1})=\{y\in [K] \mid  V(X_{n+1},y)\leq\hat{\eta}\}$.

% Traditional CP is model-agnostic, %uncertainty quantification method, 
% as it only requires prediction from the base model. %during the process.
% Moreover, various non-conformity scores can be used to instantiate the framework~\citep{romano2020classification,angelopoulos2020uncertainty}.
% % In this work, we focus on adaptive conformal prediction methods, which guarantee conditional coverage~\citep{romano2020classification,angelopoulos2020uncertainty}. 
% For instance, the Adaptive Prediction Set (APS)~\cite{romano2020classification}, the most classical adaptive conformal prediction approach, %\lizn{one-sentence summary}.
% %For any given data point $(x, y)$, APS 
% first sorts the predicted results in descending order, i.e., $\hat{\pi}_{(1)}(x) \ge \hat{\pi}_{(2)}(x) \ge \cdots \ge \hat{\pi}_{(k)}(x)$. 
% The non-conformity score is then defined by the cumulative probabilities from the most likely class to the observed class $y$ in the calibration step, i.e., $V(x,y)=\sum_{i=1}^y \hat{\pi}_{(i)}(x)$. 

%\subsection{Background}\label{sec:background}

For any natural number $n$, we write $[n]:=\{1, \ldots, n\}$.
%
We work with the most widely-used version of conformal prediction, i.e., \emph{split} conformal prediction, where we assume a calibration set $\mathcal{D}=\{(X_i,Y_i)\}_{i=1}^N$ of i.i.d. (or simply exchangeable) observations sampled from an (unknown) distribution $P_{XY}$. In standard classification, $X_i\in \mathcal{X}$ represents the input feature from a feature space $\mathcal{X}\subseteq\mathbb{R}^d$ and $Y_i \in [L]$ is a categorical label. 
A given classifier $\hat{f}$ is trained (on a training set) to predict the conditional distribution $P(Y \given X)$. Furthermore, $X_{N+1}$ is a test instance with an unknown label $Y_{N+1}$ sampled by $P_{XY}$.
%
%A core goal %of split conformal prediction~\citep{vovk2005algorithmic} is 
%to provide rigorous, distribution-free uncertainty quantification for arbitrary black-box ML models by 
CP constructs a prediction set $C(X_{N+1})$ for  $Y_{N+1}$ based on $\mathcal{D}$. 
The output $C(X_{N+1})$ guarantees marginal coverage at a user-specified level, i.e.,
%
\[
\mathbb{P}[Y_{N+1} \in C(X_{N+1})] \geq 1 - \alpha,
\]
where $\alpha\in (0,1)$ is a predefined miscoverage rate. 

%In order to construct $\hat{C}(X_{N+1})$ satisfying the above equation, classic conformal prediction methods~\citep{vovk2005algorithmic,romano2020classification} 
Typically, CP proceeds in three steps: 
(1) computing the predefined conformity score $V(x_i,y_i)$ for each sample $(x_i,y_i)\in\mathcal{D}$ using the predictive results of the classifier $\hat{f}$; 
(2) setting $(1-\alpha)(1+1/N)$-quantile score of $\mathcal{D}$ as a threshold $\hat{\eta}$; 
(3) constructing the prediction set $C_\frak{m}(X_{N+1},\mathcal{D}):=\{y\in [K] \given V(X_i,y)\geq \hat{\eta}\}$, which is used as $C(X_{N+1})$ for $X_{N+1}$. %\tl{why there is an m here?}
%Finally, we usually treat the prediction set $\hat{C}\frak{m}(X_{N+1},\mathcal{D})$ as  $\hat{C}(X_{N+1})$.

%Previous work~\citep{vovk2005algorithmic} rigorously 
It can be shown that $C_\frak{m}(X_{N+1},\mathcal{D})$ meets the desirable \emph{marginal coverage}. % on the random sample set $\{(X_i,Y_i)\}$, as well as the calibration set $\mathcal{D}$. 
Intuitively, marginal coverage implies that the prediction set is guaranteed to contain the true label with the \emph{average} $1-\alpha$ probability over the population. 
However, this guarantee is deemed to be insufficient, %can be insufficient to satisfy actual needs, 
especially when miscoverage exhibits systematic bias, disproportionately affecting individuals belonging to groups characterized by certain features.  
% \tl{this sounds a weird term}.
% the coverage errors are systematically distributed across the population—for instance, when inaccuracies disproportionately affect certain subgroups defined by specific feature values.

%Therefore, we further require 
%The strengthened 
By contrast, \emph{conditional coverage} requires $\mathbb{P}[Y_{N+1} \in C(X_{N+1}) \given X_{N+1}=x] \geq 1 - \alpha$ for each $x\in \mathcal{X}$.  
This is much stronger %notion of validity, 
as it demands correct coverage across all regions of the feature space, not just on average. However, achieving conditional coverage is impossible % in finite-sample settings without making strong distributional assumptions, and attempts to enforce it often lead to excessively conservative prediction sets.
without imposing extra assumptions on the underlying distribution $P_{XY}$ (such as %relying on 
the smoothness of $P_{XY}$~\citep{cai2014adaptive,lei2014distribution} and strictly limiting the size of feature space $\mathcal{X}$~\citep{lee2021distribution}). As these strong assumptions are often violated, conditional coverage is less meaningful in practice.
%
%This would achieve consistent coverage for every test instance $X_{N+1}$. %, regardless of its features. %Namely,  for all $x\in\mathcal{X}$ in addition to marginal coverage. 
% However, it would not be possible %to achieve %the attainment of this equality is impossible 
% without imposing extra assumptions on the underlying distribution $P_{XY}$, such as %relying on 
% the smoothness of $P_{XY}$ \citep{cai2014adaptive,lei2014distribution} and strictly limiting the size of feature space $\mathcal{X}$ \citep{lee2021distribution}. As these strong assumptions are often violated %(or: do not hold) 
% in practice, exact conditional coverage is generally unachievable.
 
Equalized coverage~\citep{romano2020malice} represents a pragmatic compromise   %between the extremes of marginal and conditional coverage, aiming 
to ensure validity across \emph{predefined} sample groups that need to be protected. 
Given a group $\mathcal{G}\subseteq \mathcal{X}$, %is one of these groups worthy of attention, 
% the indicator function  $\mathbf{1}_{\mathcal{G}}$ is defined by $\mathbf{1}_{\mathcal{G}}(x)=1$ if $x\in \mathcal{G}$, and $\mathbf{1}_{\mathcal{G}}(x)=0$ otherwise.
%Formally, we assume the training and test samples $\{(X_i, Y_i)\}_{i=1}^N$ are exchangeable draws from an arbitrary and unknown distribution $P_{XY}$, and 
it is required that %the prediction set $\hat{C}(X_{n+1})$ satisfies %the following property:
%
\begin{equation*}
\mathbb{P}[Y_{N+1} \in C(X_{N+1}) \given X_{N+1}\in \mathcal{G}] \geq 1 - \alpha
\end{equation*}
for all $\mathcal{G}$ of interest. 
In particular, these groups are typically related to some specific features called sensitive features.

However, the requirement for rigorous equalized coverage is localized, as algorithmic biases disproportionately affect only a minority of subgroups~\citep{zhou2024conformal}, as mentioned in Seciton~\ref{sec:intro}.
Therefore, AFCP further proposes adaptive equalized coverage based on equalized coverage, formalized by
\begin{equation}\label{Eq:Adaptive equalized coverage}
\mathbb{P}[Y_{N+1} \in C(X_{N+1}) \given X_{N+1}\in \hat{\mathcal{G}}] \geq 1 - \alpha,
\end{equation}
where $\hat{\mathcal{G}}$ is adaptively selected corresponding to sensitive features.
Eq.~\ref{Eq:Adaptive equalized coverage} indicates that $C(X_{N+1})$ is well-calibrated for the selected group $\hat{\mathcal{G}}$ defined by these sensitive features.



% and all $x\in \mathcal{X}$. % \tl{define G}
% where the group identifier $\mathbf{1}_{\mathcal{G}}(X)$ is an an indicator function defined by $\mathbf{1}_{\mathcal{G}}(X) = 1$ if $X\in \mathcal{G}$, and $\mathbf{1}_{\mathcal{G}}(X) = 0$ otherwise.
%
% \tl{is this not just $\mathbb{P}[Y_{N+1} \in \hat{C}(X_{N+1}) \mid X_{N+1}\in \mathcal{G}] \geq 1 - \alpha.$ for all $\mathcal{G}$?}


% Given a classifier and data set, various groups $\mathcal{G}$ usually suffer from different degrees of algorithmic bias, and the groups that need to be protected (characterized by the poor conditional coverage) are typically unknown in real-world applications. 
% Therefore, we next introduce \name .

% In practice, for a given model and data set, different groups may not exhibit the same need for rigorous equalized coverage guarantees (2), as conformal predictions may be able to approximately achieve the desired coverage even without explicit constraints. Algorithmic bias typically affects only a minority of the population, so standard prediction sets with marginal coverage (1) may approximately satisfy (2) for most groups. Therefore, we propose Adaptively Fair Conformal Prediction (AFCP), a new method that efficiently identifies and addresses groups suffering from algorithmic bias in a data-driven way, adjusting their prediction sets to equalize coverage without sacrificing informativeness.
 


% \tl{need to introduce AFCP, to determine how to write after the intro}
% \xsr{in introduction?}



==> iclr2026-3/030_method.tex <==


This section presents \name, a learning-based method that adaptively identifies groups affected by algorithmic bias and adjusts their prediction sets to achieve equalized coverage while preserving high informativeness.


\subsection{Learning Representation-Based Groups}\label{sec:learning groups}
\noindent\textbf{Optimization Objective.}
%To better express our method later, we first %define 
%
For any feature $x\in \mathcal{X}$, we write its encoding $z=f(x)\in \mathcal{Z}$, where $\mathcal{Z}$ is a latent representation space.  
%the encoding $Z$, which is determined by $f(X)$, 
Intuitively, $z$ denotes the latent representations of feature combinations of $x$. 
We introduce a random %indicator 
binary variable $S$ and $Z$ taking values in $\mathcal{Z}$ to formalize the membership of a group. Naturally, we consider a conditional distribution $P(S \given Z)$ %$S$ is governed by a Bernoulli distribution conditioned on $f(x)$. Namely, 
such that the probability of $x\in \hat{\mathcal{G}}$ for a group $\hat{\mathcal{G}}$ is equal to $\mathbb{P}(S=1\given Z=f(x))$.
%such that $S=1$ if $X\in \hat{\mathcal{G}}$; otherwise $S=0$. Then, we assume
% which conforms to a Bernoulli distribution, 
% \begin{equation}\label{Eq:S}
%  S \sim P_{S\given Z=f(X)},
% \end{equation}
%where the encoding $Z$, which is determined by $f(X)$, denotes the latent representations of feature combinations %about $\hat{\mathcal{G}}$ and 
%the   conditional distribution $P_{S\given Z}$ is a Bernoulli distribution. %with the probability $\mathbb{P}(S=1\given Z)$. 
%
% \hide{
% To further enhance the explainability of our method (mining the exact features), we introduce the encoding $Z=f(X)$ to denote latent representations of feature combinations, and 
% we apply $Z$ to effectively predict $P_{S\given Z}$ via filtering out useless feature information. Concurrently, for the sake of explainability, we also hope $Z$ can reconstruct $X$ to help us understand which features we actually choose from $X$.
% % thus we obtain $P_{S\given X}=P_{S\given Z}P_{Z\given X}$ because $Z$ merely relies on $X$.
% % When we respectively compute $P_{S\given Z}$ and $P_{Z\given X}$, the latent representations $Z$ help us figure out the reason why sample $X$ is selected.
% % and $Z_i=f(X_i)$ denotes feature combination representations of $X_i$ determined by a function $f$. 
% % \tl{I might be wrong but I think we are confusing ourselves with redundant notations, $S_i$ is **essentially** just for $H_i$?}
% % In this formalization, AFCP is a special case of Eq.~\ref{Eq:H} when $f$ is an identity function and $\mathbb{P}(S=1 \given X)$ is equal to $\mathbf{1}_{\hat{\mathcal{G}}}(x)$ for all $x\in \mathcal{X}$. 
% % \tl{it is unclear how to get the formulation of AFCP (like $\phi$ etc from $f$ being an identity. maybe elaborate, as likely the author of AFCP will review this paper}
% }
%We take an information-theoretic perspective on deep networks. 
%In addition to predicting $S$, we also care about the explainability of the selected group $\hat{\mathcal{G}}$. For this sake, we reconstruct $X$ using the encoding $Z$ to figure out which features we actually choose.
Our goal is twofold: (1) to learn an encoding $Z=f(X)$ that is maximally informative about $S$ and $X$, while (2) %simultaneously 
%to restrict the information 
$Z$ %contains about the 
does not reveal the identity of any individual $i$ in the sample (e.g., the calibration set). %$x\in \mathcal{X}$. %data point $(i)$.

We apply the \emph{deep variational information bottleneck} (Deep VIB) method~\citep{alemi2016variational}. 
Specifically, for two random variables $X$ and $Y$ with the joint pdf (parameterized by $\theta$), $p_\theta(x,y)$, $I(X,Y;\theta)=\int p_\theta(x,y)\log\frac{p_\theta(x,y)}{p_\theta(x)p_\theta(y)}~dxdy$ denotes their mutual information. The optimization objective can be formalized as
%
\begin{equation*}
\max I(Z,S;\theta) + I(Z,X;\theta) - \beta I(Z,i;\theta),
\end{equation*}
% \tl{the i should be $X$?}
where $i$ is a random variable to take any instance from the sample (e.g., in this paper, the calibration set $\mathcal{D}$) with a uniform distribution, $\theta$ is the model parameter, and $\beta$ is a weight hyperparameter. (We abbreviate $I(Z,S),I(Z,X),I(Z,i)$ as $I_1,I_2,I_3$ for convenience.)

By introducing $q_\phi(s|z),q_\varphi(x|z),r(z)$ as the variational approximation to $p_\theta(s|z),p_\theta(x|z),p(z)$ in respective terms, we perform variational inference %on the above equation 
and obtain
%
\begin{equation*}
\begin{aligned}
I_1 + I_2 - \beta I_3 &\geq \int p_\theta(x)p_\theta(s \given x)p_\theta(z \given x)\log q_\phi(s \given z) \d x \d s \d z \\
&\quad + \int p_\theta(x)p_\theta(z \given x)\log q_\varphi(x \given z) \d x \d z - \frac{\beta}{N}\sum_i\int p_\theta(z \given x_i)\log \frac{p_\theta(z \given x_i)}{r(z)}\d z.
\end{aligned}
\end{equation*}
(The details %derivation process 
are given in Appendix~\ref{appendix:var}.)


In practice, we can approximate $p_\theta(x,s)=p_\theta(x)p_\theta(s|x)$ and $p_\theta(x)$ using the empirical distribution on the observations (e.g., the calibration set $\mathcal{D}$). 
%
%
As for $p_\theta(z|x)$, the reparameterization trick~\citep{kingma2013auto} forces $z$ to conform to a normal distribution which relies on $x_i$, and hence its deterministic function %in Eq.~\ref{Eq:S} 
can be rewritten as $z=f(x,\epsilon)$ with an (auxiliary) noise variable $\epsilon$. 
% In this way, we have $p_\theta(z\given x)dz=p_\theta(\epsilon)d\epsilon$.

Substituting all of these into the above equation, we obtain the following loss function 
%
\begin{equation}\label{Eq:Loss Funciton_1}
\mathcal{L} = -\frac{1}{N}\sum_{i=1}^N \left( \mathbb{E}_{\tilde{z}\sim f(x_i,\epsilon)}[\log q_\phi(s_i\given \tilde{z}) + \log q_\varphi(x_i\given \tilde{z})] - \beta D_{\mathrm{KL}}(p_\theta(z \given x_i)\Vert r(z))\right).
\end{equation}
%\tl{what is  r(Z)?}
% \begin{equation}\label{Eq:Loss Funciton_1}
% \begin{aligned}
% \mathcal{L} &\approx -\frac{1}{N}\sum_{i=1}^N \mathbb{E}_{z\sim f(x,\epsilon)}[\log q_\phi(s_i\given z)] + \mathbb{E}_{z\sim f(x,\epsilon)}[\log q_\varphi(x_i\given z)] - \beta p_\theta(Z\given x_i)\log \frac{p_\theta(Z\given x_i)}{r(Z)} \\
% &= -\frac{1}{N}\sum_{i=1}^N \mathbb{E}_{\epsilon\sim p_\theta(\epsilon)}[\log q_\phi(s_i\given f(x_i,\epsilon)) + \log q_\varphi(x_i\given f(x_i,\epsilon))] - \beta D_{KL}(p_\theta(Z\given x_i)\Vert r(Z)).
% \end{aligned}
% \end{equation}
% where $D_{KL}$ denotes the Kullback Leibler divergence.

Intuitively, the expected log-likelihood $\mathbb{E}_{\tilde{z}\sim f(x_i,\epsilon)}[\log q_\phi(s_i\given \tilde{z}) + \log q_\varphi(x_i\given \tilde{z})]$ allows the encoding $\tilde{z}$ to predict $s_i$ and regenerate $x_i$ simultaneously, whereas the Kullback-Leibler (KL) divergence aims to compress the remaining useless information of $\tilde{z}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{Instantiation.}
Eq.~\ref{Eq:Loss Funciton_1} %, we naturally 
suggests a natural design of the Encoder-Decoder architecture. 
%
In our method, the stochastic encoder with parameter $\theta$ has the form $p_\theta(z\given x)=\mathcal{N}(z\given f_\mu(x), f_\sigma(x))$, where $f_\mu(x)$ and $f_\Sigma(x)$ are two MLP networks to output the mean and variance of a normal distribution. We set $r(z)$ as a standard normal distribution $\mathcal{N}(0,1)$ and directly minimize the KL divergence term in Eq.~\ref{Eq:Loss Funciton_1} using the reparameterization trick.

% \hide{
% Specifically, an encoder $p_\theta(z\given x)$ encodes $x$ into a stochastic representation $z$, and two different decoders $q_\phi(z)$ and $q_\varphi(z)$ are applied to predict the distribution of $s$ and reconstruct $x$ for explainability, respectively. 
% For the encoder, .\xsr{revise}
% }

We now concentrate on two decoders with parameters $\phi$ and $\varphi$. 
The instantiation of decoder with parameter $\varphi$ is trivial. For the expected log-likelihood $\mathbb{E}_{\tilde{z}\sim f(x_i,\epsilon)}[\log q_\varphi(x_i\given \tilde{z})]$ in Eq.~\ref{Eq:Loss Funciton_1}, we utilize the standard Mean Squared Error (MSE) as the reconstruction loss~\citep{kingma2013auto}.

Decoder with parameter $\phi$ aims at predicting $S$, %the condition distribution $P_{S\given Z}$ for $S$. Recall that $S$ %is an indicator variable to decide 
which indicates whether the sample $X$ belongs to group $\hat{\mathcal{G}}$ or not.
Assume %Suppose there exists a series of 
a set of observations, e.g., %as the training set, and we take 
the calibration set $\mathcal{D}=\{(X_i,Y_i)\}_{i=1}^N$. % as an example as follows. %in the following content. 
The distribution $P(S\given X)$ %in Eq.~\ref{Eq:S} 
can be viewed as a binary classifier $h$ comprising an encoder with parameter $\theta$ and a decoder with the parameter $\phi$. 
%The classificaiton 
The result of $h$ on $\mathcal{D}$ is a vector $\mathbf{s}=[s_1,\dots,s_N]\in \{0,1\}^N$. 
Let $\hat{\mathcal{G}}_\mathbf{s}\subseteq \mathcal{D}$ %\tl{technically, $\hat{\mathcal{G}}_\mathbf{s}\subseteq $ a projection of $D$ onto features?} 
denote the group determined by $\mathbf{s}$ on $\mathcal{D}$ and 
$\mathcal{H}$ be the family of all plausible $h$.
%
We extend an inequality~%(24) in 
\citep{cauchois2021knowing} %to an arbitrary nonlinear classifier, to 
to measure the deviation between the empirical coverage probability $\mathbb{P}_n$ on $\mathcal{D}$ and the oracle coverage probability $\mathbb{P}$.

\begin{proposition} \label{prop:finite}
Let the VC-dimension $VC(\mathcal{H})\leq R$ and $\delta=\lvert \hat{\mathcal{G}}_\mathbf{s} \rvert / N$ be the proportion of $\hat{\mathcal{G}}_\mathbf{s}$ to the entire dataset. Then the gap between the empirical coverage probability $\mathbb{P}_n$ on the observations and the oracle coverage probability $\mathbb{P}$ is upper bounded, i.e., there exists some constant $C_1$ for all $\tau > 0$ 
\begin{equation*}
\sup_{h\in\mathcal{H}}\left\{\lvert \mathbb{P}_n[Y \in C(X) \given X \in \hat{\mathcal{G}}_\mathbf{s}] - \mathbb{P}[Y \in C(X) \given X \in \hat{\mathcal{G}}_\mathbf{s}] \rvert \right\}  \leq C_1\sqrt{\frac{R\log N + \tau}{\delta N}}
\end{equation*} 
holds with probability at least $1-e^{-\tau}$.
\end{proposition}

Proposition~\ref{prop:finite} (cf.~Appendix~\ref{A:prop1} for proof) highlights two key directions for reducing the discrepancy between $\mathbb{P}_n$ and $\mathbb{P}$. First, a lower VC-dimension $VC(h)$ leads to a more precise estimation $\mathbb{P}_n$, implying that the classifier $h$ should exhibit limited complexity. Second, the selected group must be sufficiently large to ensure reliable estimation.

We maximize the expected log-likelihood $\mathbb{E}_{\tilde{z}\sim f(x_i,\epsilon)}[\log q_\phi(s_i \given \tilde{z})]$ in Eq.~\ref{Eq:Loss Funciton_1} via minimizing the expected empirical conditional coverage of the selected group $\hat{\mathcal{G}}$. %In Eq.~\ref{Eq:S}, 
The group $\hat{\mathcal{G}}$ on %the calibration set 
$\mathcal{D}$ is determined by a random vector $\mathbf{S}$, sampled from a joint Bernoulli distribution $B= \prod_{i=1}^N \operatorname{Bernoulli}(q_\phi(S_i=1 \given \tilde{z}))$.  
Hence, given $\mathcal{D}$, we formulate the following optimization problem :
%
\begin{equation}\label{Eq:minimize coverage}
\min_\phi \mathbb{E}_{\mathbf{S}\sim B}[\mathbb{P}_n[Y \in C(X) \given X \in \hat{\mathcal{G}}_\mathbf{S}]] \quad \text{s.t.} ~~\frac{1}{N}\sum_{i=1}^Nq_\phi(S_i=1 \given \tilde{z}) \geq \delta.
% = \frac{\lvert \hat{\mathcal{G}}_\mathbf{s} \rvert}{N}. 
% \quad q_\phi(s_i\given z) \in [0,1]. 
\end{equation}
%
In the above minimization problem, $\delta=\lvert \hat{\mathcal{G}}_\mathbf{s} \rvert/N$ denotes the the proportion of the selected group size to the whole dataset $\mathcal{D}$, and the decoder with parameter $\phi$ is a simple logistic regression model of the form $q_\phi(s \given \tilde{z})=\sigma (s\given f_m(\tilde{z}))$, where $\sigma$ is the sigmoid function and $f_m$ is a MLP network.

% \textcolor{red}{
To solve the constrained optimization problem, we employ the Projected Gradient Descent (PGD), an iterative optimization algorithm~\citep{madry2017towards}, to optimize the parameter $\phi$.
In each training step, PGD performs a gradient descent update and then projects the new point onto the feasible set to ensure all constraints are satisfied.
% } 
Specifically, when the predictive distribution $q_\phi(s\given \tilde{z})$ does not meet the constraint $ \frac{1}{N}\sum_{i=1}^Nq_\phi(S_i=1\given \tilde{z}) \geq \delta$ after one back propagation process, we project it back onto the constraint-friendly space. 
Such a projection is equivalent to an $\ell_2$ distance minimization problem. Let $q_\phi^*(s_{1}\given \tilde{z}) \geq \dots\geq q_\phi^*(s_{N}\given \tilde{z})$ be the descending order of $\{q_\phi(s_i\given \tilde{z})\}_{i=1}^N$, and  the projection results in %can be written as 
% \begin{equation}
% \begin{aligned}
% q_\phi'(s_i\given z) &= \min(1,q_\phi(s_i\given z)+\frac{\omega}{2})\\
%  &=  \min(1,q_\phi(s_i\given z)+\frac{\delta-k-\sum_{i=k+1}^Nq_\phi^*(s_{i}\given z)}{N-k})
% \end{aligned}
% \end{equation}
\begin{equation}\label{Eq:project}
q_\phi'(s_i\given \tilde{z}) = \min\left(1,q_\phi(s_i\given \tilde{z})+\frac{\omega}{2}\right),
\end{equation}
where $\omega = (\delta-k-\sum_{i=k+1}^Nq_\phi^*(s_{i}\given \tilde{z}))/ (N-k) \geq 0$, $k\in [N]$ is the greatest index to satisfy $q_\phi^*(s_{k}\given \tilde{z})+\omega/2\geq 1$ and $q_\phi^*(s_{k+1}\given \tilde{z})+\omega/2< 1$.
(The details are given in Appendix~\ref{A:opt}.)

Overall, we employ the empirical conditional coverage loss $\mathcal{L}_{\mathrm{CC}}$, the reconstruction loss $\mathcal{L}_{\mathrm{MSE}}$, and the KL divergence loss $\mathcal{L}_{\mathrm{KL}}$ to replace the corresponding terms in Eq.~\ref{Eq:Loss Funciton_1}, resulting in 
\begin{equation}\label{Eq:Loss Funciton_2}
\mathcal{L} = \mathcal{L}_{\mathrm{CC}} +  \mathcal{L}_{\mathrm{MSE}} - \beta\mathcal{L}_{\mathrm{KL}}.
\end{equation}
% \begin{equation}
% q_\phi'(s_i)= \min(1,q_\phi(s_i)+\frac{\delta-k-\sum_{i=k+1}^Nq_\phi(s_{i}^\#)}{N-k}),
% \end{equation}
% \begin{equation*}
% \mathcal{L} = \sum_{i=1}^N(v_i-u_i)^2 + \sum_{i=1}^N\lambda_i(-v_i) + \sum_{i=1}^N\mu_i(v_i-1) + \omega(\delta-\sum_{i=1}^Nv_i),
% \end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Constructing the Adaptive Prediction Sets}\label{sec:Constructing}

% \textcolor{red}{
After selecting the unfair group $\hat{\mathcal{G}}$, we proceed to construct the final prediction set with $\hat{\mathcal{G}}$. First, a standard conformal prediction set $C_\frak{m}(X_{N+1},\mathcal{D})$ is constructed using classic adaptive conformal prediction. Then, we perform $T$ sampling of the vector $\mathbf{s}_t$ $(t\in [T])$ from the joint Bernoulli distribution $B$ learned by models in Eq.~\ref{Eq:minimize coverage}. Each $\mathbf{s}_t$ defines a group $\hat{\mathcal{G}}_{\mathbf{s}_t}$, and such group is used as a calibration set to build a prediction set $C_\frak{m}(X_{N+1},\hat{\mathcal{G}}_{\mathbf{s}_t})$ as mentioned in Section~\ref{sec:prel}. The final prediction set for $Y_{N+1}$ is given by the union of all these sets:
% }
\hide{
% After evaluating Aˆ(Xn+1,y) by applying Algorithm 1 with placeholder label y for Yn+1 for all y ∈ [L], and selecting either an empty set or a single attribute Aˆ(Xn+1) using (7), AFCP constructs
% an adaptive prediction set for Yn+1 that satisfies (3) as follows.
After selecting the group $\hat{\mathcal{G}}$, we show how to construct prediction sets with $\hat{\mathcal{G}}$. %the groups.
%
First, we construct $C_\frak{m}(X_{N+1},\mathcal{D})$ using the classic adaptive conformal prediction. 
%as described in Section ~\ref{sec:background}. Then, 
We then repeat $T$ times to sample the vector $\mathbf{s}_t$ from the joint Bernoulli distribution $B$ in Eq.~\ref{Eq:minimize coverage}, and construct the prediction set $C_\frak{m}(X_{N+1},\hat{\mathcal{G}}_{\mathbf{s}_t})$ based on the selected group $\hat{\mathcal{G}}_{\mathbf{s}_t}$. 
Finally, %our \name 
the prediction set for $Y_{N+1}$ is given by
}
\begin{equation}\label{Eq:Construct}
C(X_{N+1})=C_\frak{m}(X_{N+1}, \mathcal{D})\cup \bigcup_{t=1}^T C_\frak{m}(X_{N+1},\hat{\mathcal{G}}_{\mathbf{s}_t}).
\end{equation}
Our approach \name is summarized in Algorithm~\ref{alg:framework}. To analyze its time complexity,
assume we have $M$ test instances and the complexity of conducting classic conformal prediction is $\mathcal{O}(N+M)$. 
Then, training the model to select groups is $\mathcal{O}(EN(\vert \theta \vert + \vert \phi \vert + \vert \varphi \vert))$, where $E$ is the number of epochs.
For all $M$ test instances, the time of selecting groups and constructing prediction sets is $\mathcal{O}(TN+TM)$.
The overall complexity of our \name is $\mathcal{O}(EN(\vert \theta \vert + \vert \phi \vert + \vert \varphi \vert) + T(N+M))$, which is 
%If we drop the constants, the time complexity can be re-written as 
$\mathcal{O}(N+M)$, disregarding constant multiplicative factors.
In contrast, the complexity of AFCP is $\mathcal{O}(N\log N+NM)$~\citep{zhou2024conformal}. %, indicating that the complexity of our algorithm is significantly lower than that of AFCP.


% $\mathcal{O}(N\log N+LNM+VK(N+LM))$
%--------------------------------------------------------
\begin{algorithm} 
\caption{The overall framework of \name.} 
\label{alg:framework}
\begin{algorithmic}[1]
\Require calibration dataset $\mathcal{D}=\{X_i,Y_i\}_{i=1}^N$; test instance with feature $X_{N+1}$; list of $K$ sensitive features; pre-trained classifier $\hat{f}$; fixed rule to compute nonconformity scores; level $\alpha\in (0,1)$; selected group size proportion $\delta$; hyperparameter $\beta$; sampling times $T$;
\Ensure prediction set $C(X_{N+1})$; selected group set $\{\hat{\mathcal{G}}_{\mathbf{s}_t}\}_{t=1}^T$.
\State Construct classic conformal prediction set $C_\frak{m}(X_{N+1},\mathcal{D})$ based on the output of $\hat{f}$;
\For {each batch}
\State Calculate KL divergence loss $\mathcal{L}_{KL}$ with reparameterization trick;
\State Sample $\tilde{z}\sim f(x,\epsilon)$;
\State Calculate conditional coverage loss $\mathcal{L}_{CC}$ and reconstruction loss $\mathcal{L}_{MSE}$ using $\tilde{z}$;
\State Put all losses together in $\mathcal{L}$ as defined in Eq.~\ref{Eq:Loss Funciton_2};
\State Update parameters $\theta,\phi$ and $\varphi$ via the gradient descent of $\mathcal{L}$; 
\If{$\sum_{i=1}^Nq_\phi(S_i=1\given \tilde{z})<\delta\cdot N$}
\State Project each $q_\phi(S_i=1\given \tilde{z})$ to satisfy minimum set constraint using Eq.~\ref{Eq:project};
\EndIf
\EndFor
\For {$t\in [T]$}
\State Sample $\mathbf{s}_t\sim B$;{\Comment{\emph{B is a joint Bernoulli distribution mentioned in Eq.~\ref{Eq:minimize coverage}}}}
\State Construct $C_\frak{m}(X_{N+1},\hat{\mathcal{G}}_{\mathbf{s}_t})$;
\EndFor
\State Construct prediction set $C(X_{N+1})$ following Eq.~\ref{Eq:Construct}.
\end{algorithmic}
\end{algorithm}
%------------------------------------------------------------

% Given a pre-trained multi-class classifier, consider a calibration dataset D of size n. Let L denote the total number of possible labels to predict, and let K denote the number of sensitive attributes. For each attribute k ∈ [K], let Vk ∈ N denote the count of its possible values. Denote V = maxk Vk as the maximum count across all attributes.

The following result, proved in Appendix~\ref{A:thm}, ensures that the prediction set $C(X_{N+1})$ generated by \name achieves adaptive equalized coverage (Eq.~\ref{Eq:Adaptive equalized coverage}) over the selected group set $\{\hat{\mathcal{G}}_{\mathbf{s}_t}\}_{t=1}^T$.

\begin{theorem}\label{thm:equalized coverage}
If $\{(X_i,Y_i)\}^{N+1}_{i=1}$ are exchangeable, the prediction set $C(X_{N+1})$ and the selected group set $\{\hat{\mathcal{G}}_{\mathbf{s}_t}\}_{t=1}^T$ output by Algorithm~\ref{alg:framework} satisfy the adaptive equalized coverage defined in Eq.~\ref{Eq:Adaptive equalized coverage},
% \textcolor{red}{
and this guarantee still holds when the selected groups are defined by a more complex combination of features (e.g., non-linear) compared to AFCP.
% }
% the candidate group space of our method serves as a superset of that of AFCP.
\end{theorem}




==> iclr2026-3/040_experiments.tex <==
\subsection{Experimental Setup}\label{sec:settings}
\noindent\textbf{Baselines.}
We select the classic CP method Marginal~\citep{romano2020classification} for classification, the initial CP method Partial~\citep{romano2020malice} considering equalized coverage, and the state-of-the-art method AFCP~\citep{zhou2024conformal} as our baselines.
The vanilla version of AFCP is designed to pick at most one sensitive feature (referred to as AFCP1). 
We also extend AFCP1 to select two sensitive features (referred to as AFCP2), given unreal, strong 
prior knowledge. Note that in real-world applications, it is typically unknown exactly how many features the unfair group may correspond to.


\noindent\textbf{Evaluation Metrics.}
To evaluate the prediction sets $C(X_{N+1})$ produced by different CP methods, we use the coverage conditional on a specific group (referred to as Group Coverage), Average Coverage (viz., marginal coverage), and Average Size (viz., efficiency) as the metrics.

Additionally, we propose a new conditional coverage metric, viz., $\text{WSC}^+$, to capture groups defined by complicated (nonlinear) feature relationships. 
Traditional conditional coverage metric~\citep{cauchois2021knowing} considers the worst coverage over all slabs containing $\delta$ mass on the observations, which is defined as
\begin{equation*}
\text{WSC}_n(C,\mathbf{v}):=\inf_{a<b}~ \left\{\mathbb{P}_n(Y\in C(X)\given a \leq \mathbf{v}^TX \leq b) ~~\text{s.t.}~~ \mathbb{P}_n(a \leq \mathbf{v}^TX \leq b) \geq \delta\right\},
\end{equation*}
where $\mathbf{v}\in \mathbb{R}^d$ and $a<b\in \mathbb{R}$.

To strengthen the %expressiveness of 
WSC metric, we replace the linear mapping $\mathbf{v}^T$ in the above equation with an 
arbitrary non-linear function $\pi$, giving rise to $\text{WSC}^+$, i.e.,
\begin{equation}\label{Eq:wsc+}
\text{WSC}^+_n(C,\pi):=\inf_{a<b}~ \left\{\mathbb{P}_n(Y\in C(X)\given a\leq \pi(X) \leq b) ~~\text{s.t.}~~ \mathbb{P}_n(a\leq \pi(X) \leq b) \geq \delta\right\}.
\end{equation}
%
Assume a quadratic function $\pi(\mathbf{x})=\mathbf{x}^T\mathbf{W}\mathbf{x}+\mathbf{v}^T\mathbf{x}$, where $\mathbf{W}\in \mathbb{R}^{d\times d}$ and $\mathbf{v}\in \mathbb{R}^d$. We uniformly draw 1,000 samples $\pi_j=\{\mathbf{W}_j,\mathbf{v}_j\}$ to compute the worst-slab coverage for each $\pi_j$ on the test instances. Following~\cite{cauchois2021knowing}, we use the grid search to achieve the optimal $a,b$ satisfying the desiderata as well.
In this case, we have a lower bound for our metric $\text{WSC}^+$.

\begin{proposition}\label{prop:metric}
Let $\pi(\mathbf{x})=\mathbf{x}^T\mathbf{W}\mathbf{x}+\mathbf{v}^T\mathbf{x}$ be a quadratic function and $\Pi$ be a parameter space of $\pi$. Then, if $C$ effectively provides conditional coverage at level $1-\alpha$, we have %should observe that  
\begin{equation}\label{Eq:wsc+ bound}
\text{WSC}^+_n=\inf_{\pi\in \Pi}~\text{WSC}^+_n(C, \pi) \geq 1-\alpha-\mathcal{O}(1)\sqrt{\frac{\mathcal{O}(d^2)\log N}{\delta N}}.
\end{equation}
\end{proposition}
The proof is given in Appendix~\ref{A:prop2}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{minipage}{0.45\linewidth}
\centering
\includegraphics[width=0.92\columnwidth]{figs/wsc_cdf.pdf}
\vspace{-0.7em}
\caption{
% \textcolor{red}{
CDF of Conditional Coverage ($\delta=0.5$), which plots the respective cumulative probability curves of different worst-slab coverage discovered by $\text{WSC}_n(C,\mathbf{v})$ and $\text{WSC}_n^+(C,\pi)$ over 1,000 samplings. The red curve is always above the blue curve, indicating that our $\text{WSC}_n^+(C,\pi)$ finds more groups with the poor coverage than $\text{WSC}_n(C,\mathbf{v})$.\label{F:cdf}
% }
% CDF of Conditional Coverage ($\delta=0.5$). $\text{WSC}_n^+(C,\pi)$ finds more groups with the poor coverage than $\text{WSC}_n(C,\mathbf{v})$.\label{F:cdf}
}
\end{minipage}
\hfill
\begin{minipage}{0.53\linewidth}
\centering
\vspace{4pt}
\resizebox{\linewidth}{!}{
\begin{sc}
\begin{tabular}{lccccc}
\toprule
{Metric} & $\delta=0.1$ & $\delta=0.2$  & $\delta=0.3$ & $\delta=0.4$ & $\delta=0.5$ \\
 \midrule
\multirow{2}*{$\text{WSC}_n$} & 0.616 & 0.748 & 0.793 & 0.822 & 0.842 \\
    & (0.053) & (0.037) & (0.025) & (0.023) & (0.023) \\
\midrule
\multirow{2}*{$\text{WSC}^+_n$} & 0.582 & 0.674 & 0.750 & 0.800 & 0.829 \\
     & (0.047) & (0.048) & (0.034) & (0.028) & (0.024) \\
\midrule
Imp. & -5.52\% & -9.89\% & -5.42\% & -2.68\% & -1.54\%  \\
\bottomrule
\end{tabular}
\end{sc}}
\vspace{8pt}
\captionof{table}{
% \textcolor{red}{
Performance of $\text{WSC}_n$ and $\text{WSC}_n^+$ metrics w.r.t. different $\delta$. We repeat the experiment 10 times, and report the average results (the value in () is the standard deviation). Smaller coverage is better. Our metric $\text{WSC}^+_n$ performs better than $\text{WSC}_n$ by up to $9.89\%$ to mine the group with the minimum worst-slab
coverage (defined in Eq.~\ref{Eq:wsc+ bound}).
% }
% The Worst Slab Coverage w.r.t. different $\delta$. Smaller coverage is better. The metric $\text{WSC}^+_n$ performs better than $\text{WSC}_n$.
}
\label{T:class condition distance}
\end{minipage}  
\vspace{-0.8em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To demonstrate the advantages of the new metric $\text{WSC}^+$, we randomly draw the features $X\in [0,1]^{10}$ from a uniform distribution and create a simple dataset for classification as described in Appendix~\ref{A:hyperparameter}. 
Note that we define the group needed to be protected to satisfy $(X[0]\geq0.1)\oplus(X[1]\geq0.1)=\text{True}$.
We respectively plot the Cumulative Distribution Functions (CDF) of $\text{WSC}_n(C,v)$ and $\text{WSC}^+_n(C,\pi)$ over 1,000 samples $\pi_j$ when $\delta=0.5$ in Fig.~\ref{F:cdf}, and observe that our $\text{WSC}^+_n(C,\pi)$ always reveals the groups with the worse coverage than that of $\text{WSC}_n(C,v)$, which can be attributed to %This performance benefits from the powerful 
representational capability of the nonlinear function $\pi$ in $\text{WSC}^+_n(C,\pi)$.

Moreover, we also list the average results of two metrics, $\text{WSC}_n$ and $\text{WSC}^+_n$, as $\delta$ increases over 10 repeated experiments in Table~\ref{T:class condition distance}.
Similar to Fig.~\ref{F:cdf}, the minimum worst-slab coverage found by our $\text{WSC}_n^+$ is smaller than that found by  $\text{WSC}_n$ by up to $9.89\%$. As $\delta$ increases, the condition coverage tends to the marginal coverage (0.9), and the gap between $\text{WSC}_n$ and $\text{WSC}_n^+$ narrows, as expected.


\hide{
Moreover, we also list the results of $\text{WSC}_n$ and $\text{WSC}^+_n$ as $\delta$ increases in Table~\ref{T:class condition distance}.
Similar to Fig.~\ref{F:cdf}, the worst-slab coverage found by $\text{WSC}_n^+$ is smaller than that found by  $\text{WSC}_n$ by up to $9.89\%$. As $\delta$ increases, the condition coverage tends to the marginal coverage (0.9), and the gap between $\text{WSC}_n$ and $\text{WSC}_n^+$ narrows, as expected. %becomes slight.
% In each of our coming experiments, we set $\delta=0.5$ of $\text{WSC}_n^+$ by default.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{Implementations.}\footnote{Our code is publicly available at https://github.com/Xusr1123/FaReG.}
% \footnote{An implementation of our approach can be accessed at the following anonymous link: https://github.com/Anonymity67543/FaReG.}
All the experiments are carried out on NVIDIA GeForce RTX 3090. We repeat each experiment 10 times and report the average to suppress randomness. 
We set $\delta=0.5$ for $\text{WSC}_n^+$ by default. More implementation details, such as hyperparameters and training settings, are presented in Appendix~\ref{A:hyperparameter}.
% An implementation of our approach is available at \url{https://github.com/Anonymity67543/FaReG}.


\subsection{Synthetic Data}\label{sec:synthetic data}

We evaluate our method on synthetic data designed to mimic a mental illness diagnosis scenario. The dataset includes six possible labels: Depression, Anxiety Disorders, Bipolar Disorder, Schizophrenia, Anorexia, and Post-Traumatic Stress Disorder (PTSD).
Each sample contains four sensitive features—Age Group, Region, Gender, and Color—along with six non-sensitive features independently sampled from a uniform distribution within a value range $[0,1]$. The sensitive features are generated as follows:
(1) Gender is uniformly drawn from \textit{\{Female, Male\}};
(2) Color is uniformly drawn from \textit{\{Red, Blue\}};
(3) Age Group is drawn from \textit{\{Child, Youth, Middle, Elder\}} with equal probability;
(4) Region follows a fixed cyclical sequence: Asia, Europe, Africa, America, Oceania.

We then generate true labels $Y$ for the dataset, where diagnosis is more challenging for a specific subgroup defined by the Exclusive NOR (XNOR) operation (cf. Appendix~\ref{A:hyperparameter}).
Specifically, we assume $X[0]$ is Color, $X[1]$ is Gender, and $X[2]$ is any non-sensitive feature, and define $Y$ based solely on these three attributes. Through the label generation, we have the following subgroup $X[0]\odot X[1]=\textit{True}$: \textit{Color=Red (True) \& Gender=Female (True)} or \textit{Color=Blue (False) \& Gender=Male (False)}, simulating a real-world situation that algorithmic biases occur on this subgroup.
%For notational simplicity, we let $X[k]$ denote the $k$-th feature. We assume $X[0]$ is Color, $X[1]$ is Gender, and $X[2]$ is any non-sensitive feature. %the first standard feature).
% The true label $Y$ is generated by a decision tree model (cf. Appendix~\ref{A:hyperparameter}) that depends solely on $X[0]$, $X[1]$ and $X[2]$. This design intentionally creates a scenario where diagnosis is more challenging for two specific subgroups defined by the Exclusive NOR (XNOR) operation $X[0]\odot X[1]=\textit{True}$: \textit{Color=Red (True) \& Gender=Female (True)} or  \textit{Color=Blue  (False) \& Gender=Male (False)}, simulating a real-world situation that algorithmic biases may occur.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{\textwidth}
        \centering
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/Conditional_Coverage_comparison.pdf}
            % \vskip -0.3em
            \caption{Group Coverage}\label{F:exp1_1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/WSC_comparison.pdf}
            % \vskip -0.3em
            \caption{$\text{WSC}^+_n$}\label{F:exp1_2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/Coverage_comparison.pdf}
            % \vskip -0.3em
            \caption{Average Coverage}\label{F:exp1_3}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/Average_Size_comparison.pdf}
            % \vskip -0.3em
            \caption{Average Size}\label{F:exp1_4}
        \end{subfigure}
        \vskip -0.5em
        \caption{Performance of prediction sets produced by different CP methods on synthetic data w.r.t. the total number of training and calibration data instances. 
        Only our \name achieves the ideal conditional coverage (0.9), and meanwhile, does not sacrifice too much information (set sizes) compared to baselines.  \label{F:exp1}
        }
    \end{minipage}
\end{figure}


% \input{tables/time.tex}
%+===================
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{\textwidth}
        \centering
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/time_cost_comparison.pdf}
            % \vskip -0.3em
            \caption{Time Cost}\label{F:time}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/custom_attribute_selection_8.pdf}
            % \vskip -0.3em
            \caption{Selects $X[0]$}\label{F:attr8}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/custom_attribute_selection_9.pdf}
            % \vskip -0.3em
            \caption{Selects $X[1]$}\label{F:attr9}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/custom_attribute_selection_8_9.pdf}
            % \vskip -0.3em
            \caption{Selects $X[0] \&X[1]$}\label{F:attr8_9}
        \end{subfigure}
        \vskip -0.5em
        \caption{Fig.~(a) reports the running time of different CP methods with the increasing total number of training and calibration data instances. 
        % Our method significantly outperforms the baselines. 
        Fig.~(b)--(d) are the results of the selection frequency of target features $X[0]$ and $X[1]$.
        As the sample size increases, our method becomes more consistent with target features.}
        \label{F:exp2}
    \end{minipage}
\end{figure}
%+===================


% \input{tables/condition_per_efficiency_1}

\hide{
% In this part, we evaluate the performance of \name on synthetic data that mimic a mental illness diagnosis scenario with six possible mental disease labels, including Depression, Anxiety Disorders, Bipolar Disorder, Schizophrenia, Anorexia, and Post-Traumatic Stress Disorder (PTSD).
% There are four sensitive features-Age Group, Region, Gender, and Color, along with six normal features independently sampled from a uniform distribution within a range $[0,1]$.
% For sensitive feature Gender, it takes values from \textit{$\{$Male, Female$\}$} with equal probability. Color gets its values from \textit{$\{$Red, Green$\}$} in the same way as Gender. Age Group is randomly drawn i.i.d. from a multinomial distribution over $\{<18, 18-40, 41-65, >65\}$ with equal probability.
% Region follows a cyclically structured sequence: Asia, Europe, Africa, America, Oceania.
% For notational simplicity, we abuse $X[k]$ to denote the $k$-th feature, e.g., $X[0]$ is Color, $X[1]$ is Gender, and $X[2]$ is the first normal feature. 
% Given a $X$, the label $Y$ is generated based on a decision tree model that depends only on $X[0]$, $X[1]$ and $X[2]$, as described in Appendix.
% As a consequence of the above design, we intentionally makes diagnosis more challenging for individuals with Color Red \& Gender Male and Color Green \& Gender Female, which mimics a real situation where algorithmic bias may occur.
}


Fig.~\ref{F:exp1} depicts the results of conditional coverage, average coverage (marginal coverage), and average prediction set size (efficiency), respectively.
For conditional coverage, Group Coverage is the coverage on the subgroups defined by XNOR operation as mentioned in data construction, and we compute $\text{WSC}^+_n$ on four predefined sensitive features.
In Fig.~\ref{F:exp1_1} and~\ref{F:exp1_2}, %contrasted with baselines, 
our \name is the only one that always achieves valid coverage (greater than 0.9) for the targeted group with varying sample sizes. 
Although the conditional coverage of AFCP2 also exceeds 0.9 when the sample size reaches 500, as shown in Fig.~\ref{F:exp1_4}, it produces considerably larger prediction sets, %significantly increases the prediction set size, which costs too useful information benefiting 
which is less informative for %the 
decision-making.

\hide{
To further demonstrate the superiority of our method, we report the increase in conditional coverage per efficiency. % as a supplement. 
Specifically, in Fig.~\ref{F:exp1_1} and~\ref{F:exp1_4}, we compute the ratio of Group Coverage difference between CP methods,  and Marginal to Efficiency difference (set size) denoted as $\Delta G/\Delta E$. Similarly, we have $\Delta W/\Delta E$ for $\text{WSC}^+_n$. 
% \tl{$\Delta W/\Delta E$?}
The results are listed in Table~\ref{T:C/E}.
We observe that our method outperforms all competitors as $N$ increases, which indicates that \name precisely captures the unfair groups with poor conditional coverage.
}

In Fig.~\ref{F:time}, we compare the average running time of different CP methods (e.g., the wall-clock time of the entire \name pipeline) over 10 repeated experiments, and \name significantly reduces the time cost. 
% whose time complexity is linear in the number of data instances. 
Actually, the training of the encoder-decoder network occupies most of the time cost (e.g., in one trial with a sample size of 2,000, the training step required 161.3 seconds, while the rest took only 0.8 seconds). Additionally, the training time of the encoder-decoder network scales linearly w.r.t the sample size since we fix the epoch number and batch size in our algorithm.
This result is consistent with the analysis in Section~\ref{sec:Constructing}.

% \textcolor{red}{
To determine which features are selected by our method, we analyze the predictive variable $S$ and the reconstructed feature $\hat{X}$ by perturbing the latent representation $Z$, following the Beta-VAE approach~\citep{higgins2017beta}. Specifically, we impose a slight perturbation (e.g., $\pm 0.001$) on each dimension of $Z$ and identify the dimension that most influences $S$. Given this influential dimension and prior knowledge (as in AFCP2) that there are exactly two target features, we compute the change ratios for each dimension of $\hat{X}$ before and after perturbation, and select the two features with the top-2 maximum change ratios.
% }

% \textcolor{red}{
Figures~\ref{F:attr8}, \ref{F:attr9}, and \ref{F:attr8_9} respectively report the frequency of selecting $X[0]$ or $X[1]$ individually, and that of selecting both $X[0]$ and $X[1]$ simultaneously. The results demonstrate that our approach captures more target features than the baselines, and this advantage becomes more pronounced as the sample size increases.
% }

\hide{
To figure out which feature \name actually chooses, we observe the predictive $S$ and reconstruction $\hat{X}$ via changing $z$, following the Beta-VAE method~\citep{higgins2017beta}. Specifically, we manually impose a slight perturbation (e.g., $\pm 0.001$) on each 
dimension of $Z$ and pick the most influential dimension to $S$. Given this dimension of $Z$ and a prior knowledge as AFCP2—there are totally two target features, we compute the differences of $\hat{X}$'s each dimension before and after perturbation, and select two features with the top-$2$ max change ratio.
Fig.~\ref{F:attr8}, \ref{F:attr9} and \ref{F:attr8_9} respectively report the frequency of  selecting $X[0]/X[1]$ solely, and that of simultaneously selecting $X[0]\&X[1]$.
It can be observed that our approach captures more target features than baselines, and this advantage is more evident when the sample size increases.
}

Additionally, we present the results of parameter sensitivity and group visualization in Appendix~\ref{A:Parameter sensitivity} and~\ref{A:vision}, respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Nursery Data}\label{sec:nursery data}

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{\textwidth}
        \centering
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/real_Conditional_Coverage_comparison.pdf}
            % \vskip -0.3em
            \caption{Group Coverage}\label{F:nursery_exp1_1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/real_WSC_comparison.pdf}
            % \vskip -0.3em
            \caption{$\text{WSC}^+_n$}\label{F:nursery_exp1_2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/real_Coverage_comparison.pdf}
            % \vskip -0.3em
            \caption{Average Coverage}\label{F:nursery_exp1_3}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/real_Average_Size_comparison.pdf}
            % \vskip -0.3em
            \caption{Average Size}\label{F:nursery_exp1_4}
        \end{subfigure}
        \vskip -0.5em
        \caption{Performance of prediction sets produced by different CP methods on the Nursery data w.r.t. the total number of training and calibration data instances. 
        Only our \name achieves the ideal conditional coverage (0.9) and keeps most of the uncertainty information of sets.
        }
        \label{F:nursery_exp2}
    \end{minipage}
\end{figure}

% \input{tables/condition_per_efficiency_2}

We evaluate our \name and baseline methods on the publicly available Nursery data~\citep{nursery_76}, originally constructed from a hierarchical decision model developed to rank applications for nursery schools. The dataset comprises 12,960 instances, each described by eight categorical features: Parents’ occupation (3 levels, $\textit{Parent:=\{usual, pretentious, great-pret\}}$), Child’s nursery (5 levels), Family form (4 levels), Number of children (4 levels), Housing conditions (3 levels), Financial standing (2 levels, $\textit{Finance:=\{convenient, inconv\}}$), Social conditions (3 levels) and Health status (3 levels). The task is to classify applications into one of five priority ranks. We take all features into account (as sensitive features) except Housing conditions.

In data preprocessing, we strictly follow~\citet{zhou2024conformal}, and consider a group defined by $\textit{Parent=usual } \& \textit{ Finance=inconv}$ or $\textit{Parent=pretentious } \& \textit{ Finance=inconv}$. 
To make the issue more interesting and control the degree of algorithmic bias, we corrupt the labels of instances in such a group by adding independent, uniform noise and rounding to the nearest integer (label) as similar as \cite{zhou2024conformal}. 
This perturbation amplifies the intrinsic unpredictability of the group defined before, thereby increasing its vulnerability to algorithmic bias.

Fig.~\ref{F:nursery_exp2} presents the results. Our method consistently achieves the valid coverage under both conditional coverage metrics, i.e., Group Coverage and $\text{WSC}^+_n$, outperforming all baselines. Partial and AFCP2 perform better than the other CP methods, but \name still achieves superior results.

==> iclr2026-3/050_related.tex <==

% %%%%%%%%%%%%%%%%%%%%%%% simply copied without adaptation. %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \noindent\textbf{Conformal Prediction.}
% Uncertainty Quantification (UQ)~\cite{abdar2021review} aims to provide calibrated uncertainty estimates for machine learning models, enabling reliable decision-making in critical applications. UQ has been widely studied in both classification and regression, where typical methods include Bayesian methods~\cite{gal2016dropout}, confidence calibration~\cite{guo2017calibration}, and model-agnostic frameworks that construct uncertainty intervals~\cite{romano2019conformalized}. However, most of these methods fail to provide rigorous statistical guarantees regarding coverage, especially in non-i.i.d. settings. %For example, although ensemble-based methods can capture epistemic uncertainty, they lack formal guarantees on the reliability of predictions. 

% CP, as a UQ method, distinguishes itself in providing guaranteed coverage, regardless of the underlying model or data distribution. %Since its inception~\cite{vovk2005algorithmic}, CP 
% It has been applied to diverse domains, including image classification~\cite{sadinle2019least}, object detection~\cite{teng2022predictive}, and large language models~\cite{kumar2023conformal}. 
% %
% Most CP methods rely on splitting the dataset into a training set and a held-out calibration set to estimate non-conformity scores, as proposed in split conformal prediction~\cite{lei2015conformal}. Other extensions, such as jackknife methods~\cite{barber2021predictive} and cross-validation-based approaches~\cite{vovk2015cross}, can further enhance CP's flexibility and applicability. 

% Some work has focused on improving the efficiency and adaptability of CP by refining non-conformity scores. Adaptive Prediction Sets (APS)~\cite{romano2020classification} introduced a score function that accumulates sorted softmax probabilities; %to construct prediction sets. %Although effective, the long-tailed distribution of softmax scores often leads to the inclusion of unnecessary classes in the prediction set. 
% Regularized Adaptive Prediction Sets (RAPS)~\cite{angelopoulos2020uncertainty} extended APS by adding penalties to tail classes and Sorted Adaptive Prediction Sets (SAPS)~\cite{huang2024conformal} substituted probability values with sort orders, both resulting in more efficient prediction sets with minimal computational overhead. On a different dimension, considerable efforts have been devoted to proving (stronger) conditional coverage. These include SCP+conditional calibration \cite{gibbs2024conformalpredictionconditionalguarantees}, randomly localized
% conformal prediction \cite{hore2024conformalpredictionlocalweights}, and posterior conformal prediction \cite{zhang2024posteriorconformalprediction}, to name a few. %\xsr{saps~\cite{huang2024conformal}}

% CP has also been explored in graph-structured data. %, where node dependencies pose unique challenges for traditional methods. 
% The first work~\cite{wijegunawardana2020node} proposed a margin-based score for graphs. Afterwards, more methods, such as NAPS~\cite{clarkson2023distribution}, DAPS~\cite{zargarbashi2023conformal}, and a Jackknife+ variant for GCNs~\cite{kang2022jurygcn}, have been developed to incorporate graph-specific properties such as homophily, further improving their performance. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Conformal prediction methods differ primarily in how they balance statistical efficiency against computational tractability. Full conformal prediction achieves exact finite-sample marginal coverage under the assumption of exchangeability, but its requirement to refit or reevaluate the model for each test instance makes it computationally prohibitive for modern large-scale models. 

% Split conformal prediction offers a practical alternative by partitioning the data into a training set and a calibration set, thereby retaining marginal coverage guarantees while greatly reducing computational cost; however, this comes at the expense of statistical efficiency, as only part of the data contributes to model fitting. 

% To mitigate the loss of efficiency, cross-conformal prediction leverages cross-validation, allowing all data to serve both training and calibration roles, though its coverage guarantee is only approximate in finite samples. More recently, approaches such as Jackknife+ have been proposed to improve efficiency while maintaining approximate coverage, particularly in regression settings, albeit with increased computational burden. Collectively, these variants illustrate the trade-off between validity, efficiency, and scalability in conformal prediction.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Conformal correction refers to the use of conformal prediction techniques to adjust the outputs of a predictive model in order to restore or improve statistical validity. Standard machine learning models produce point predictions or probabilistic scores without offering rigorous guarantees on their reliability. Conformal methods, by contrast, construct prediction regions or sets that contain the true outcome with a prescribed probability, typically ensuring finite-sample marginal coverage under the assumption of exchangeability. Conformal correction leverages this principle to “wrap around” an existing model: rather than retraining the model, it applies a calibration step—often on a held-out dataset—to adjust thresholds, quantiles, or uncertainty measures so that the resulting prediction sets achieve the desired coverage level. This correction can be applied in diverse settings, such as classification (e.g., adjusting probability scores to produce valid prediction sets), regression (e.g., correcting intervals to guarantee coverage), or structured tasks like time series and natural language processing. Importantly, while conformal correction guarantees validity in a distribution-free manner, it typically provides marginal rather than conditional coverage, and the efficiency of the resulting sets depends on the quality of the underlying model.

%============================================================
Conformal Prediction (CP) has seen vigorous development in recent years~\citep{vovk2005algorithmic,smith2024uncertainty}.
Its applications span diverse domains, from image classification~\citep{sadinle2019least} and object detection~\citep{teng2022predictive} to large language models~\citep{kumar2023conformal}.

Some CP work, building on the split conformal framework~\citep{papadopoulos2002inductive, lei2018distribution}, introduces advanced nonconformity scores to ensure valid marginal coverage on the empirical data distribution. For example, \citet{romano2019conformalized} gives a nonconformity score based on quantile regression, while \citet{romano2020classification} and \citet{angelopoulos2020uncertainty} design nonconformity scores for classification.
Additionally, \citet{hoff2023bayes} proposes a nonconformity score to achieve Bayes optimal coverage.
% Additional methodologies such as jackknife~\citep{barber2021predictive} and cross-validation-based approaches~\citep{vovk2015cross} have been developed, thereby enhancing the flexibility and applicability of conformal prediction.

Another line of work has explored various notions of equalized coverage~\citep{romano2020malice} and empirically evaluated the corresponding conformal predictors in real-world applications~\citep{lu2022fair}.
For regression tasks, \citet{wang2023equal} guarantees equal coverage rates across more fine-grained groups on continuous features, and 
\citet{liu2022conformalized} propose to learn a real-valued quantile function with respect to sensitive features.
They address a distinct notion of equalized coverage tailored to continuous outcomes.
In classification, label-conditional coverage is a common alternative to equalized coverage~\citep{vovk2003mondrian,lofstrom2015bias,ding2023class}. 
This work defines the groups to be protected based on the label $Y_{N+1}$, instead of the features $X_{N+1}$.
\citet{jung2022batch}, \citet{vadlamani2025generic},    and 
\citet{gibbs2025conformal} adopt group-conditional coverage, which is analogous to equalized coverage, to improve prediction sets.
Different from the previous work, our approach \name can adaptively identify unfairly treated groups without the assumption that such groups are pre-defined.
AFCP~\citep{zhou2024conformal} develops an algorithm to construct CP sets with valid equalized coverage for adaptively selected groups, which establishes the current state-of-the-art for equalized coverage tasks.
%\xsr{to be added ...}

% \citet{jin2025confidence}
% \citep{cherian2023statistical}
%============================================================
% writen by zyk:
\hide{
\noindent\textbf{Conformal Prediction for Guaranteed Uncertainty}
Uncertainty Quantification (UQ) is crucial for developing trustworthy machine learning systems; however, many popular methods, such as Bayesian deep learning~\cite{gal2016dropout} and model ensembles, lack rigorous statistical guarantees. Conformal Prediction (CP) distinguishes itself by providing distribution-free, finite-sample marginal coverage guarantees, regardless of the underlying model's complexity or the data distribution~\cite{vovk2005algorithmic}. This robust theoretical foundation has led to its wide adoption across diverse applications, including computer vision~\cite{sadinle2019least, teng2022predictive} and large language models~\cite{kumar2023conformal}, making it a cornerstone of modern UQ.

\noindent\textbf{The Trade-off Between Validity and Efficiency}
A central challenge in CP is striking a balance between its theoretical validity and computational and statistical efficiency. To overcome this, split conformal prediction~\cite{lei2015conformal} has become the standard practice. It achieves computational tractability by partitioning data into a single training and calibration set, but at the cost of statistical efficiency, as a portion of the data is withheld from training. Subsequent methods like cross-validation-based CP~\cite{vovk2015cross} and Jackknife variants~\cite{barber2021predictive} aim to improve data efficiency by allowing all samples to be used for both training and calibration, albeit typically providing approximate rather than exact finite-sample guarantees.

\noindent\textbf{Advancements in Set Efficiency and Adaptability}
Recent research has focused on enhancing the practicality of CP by improving the efficiency of the prediction set. Methods like Adaptive Prediction Sets (APS)~\cite{romano2020classification} and its successors, RAPS~\cite{angelopoulos2020uncertainty} and SAPS~\cite{huang2024conformal}, refine the non-conformity score to produce tighter and more informative sets with minimal overhead. Concurrently, significant effort is being directed toward strengthening theoretical guarantees from marginal to (approximate) conditional coverage~\cite{gibbs2024conformalpredictionconditionalguarantees, hore2024conformalpredictionlocalweights, zhang2024posteriorconformalprediction}.

\noindent\textbf{Fairness and Group-Conditional Coverage}
% Group-balanced conformal prediction is a refinement of conformal prediction (CP) motivated by fairness concerns.
Standard marginal coverage may mask subgroup disparities, motivating recent work on stronger group-wise guarantees, such as equalized coverage~\cite{romano2020malice, lu2022fair} and label-conditional coverage~\cite{lofstrom2015bias, ding2023class}. While effective, a critical assumption in many of these methods is that the sensitive groups are pre-defined~\cite{gibbs2025conformal, jung2022batch}. This leaves open the more challenging and practical setting where such groups are unknown and must be discovered automatically to ensure fairness. Although related methods exist for identifying group-wise disparities~\cite{cherian2024statistical} or for prediction on adaptively selected subsets~\cite{jin2025confidence}, integrating group discovery explicitly within a conformal framework to correct for algorithmic bias remains underdeveloped.
}





%============================================================
% introduce split conformal prediction, marginal and conditional coverage 
% evaluations (adapttivity: set size, conditional coverage,, feature stratified converage metric) 

==> iclr2026-3/060_conclusion.tex <==

 In this paper, we propose \name, a fair conformal prediction method that learns latent groups to achieve adaptive equalized coverage. By leveraging a variational encoder-decoder to discover subgroups wih poor coverage in a high-level feature space, our approach captures complex algorithmic biases that linear methods may neglect and can be adapted to different fairness notions. 
 We also propose $\text{WSC}^+$, a nonlinear metric for evaluating the conditional coverage of unfair groups more accurately. 
 Extensive experiments confirm that \name efficiently offers stronger fairness guarantees, showing a more expressive and practical path toward fair, reliable conformal inference.

\noindent\textbf{Limitations.} 
The enhanced expressivity of representation-based groups may 
sacrifice model interpretability partially, compared to groups explicitly defined on manifest features. 
However, the encoder-decoder structure compensates this shortcoming well via reconstructing the input $X$, which is empirically confirmed by Section~\ref{sec:synthetic data} and Appendix~\ref{A:vision}.



% This paper introduced \name, a novel conformal prediction framework that achieves adaptive equalized coverage by identifying underrepresented subgroups in a learned latent feature space. By moving beyond predefined or linear groupings, \name captures complex, non-linearly separable groups that are often sources of algorithmic bias. We also proposed $\text{WSC}^+$, a nonlinear metric for evaluating conditional coverage more accurately. Experimental results demonstrate that our method provides stronger fairness guarantees with enhanced expressiveness, offering a more reliable pathway toward equitable uncertainty quantification.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Acknowledgment}
We appreciate anonymous reviewers for their valuable comments.  
This work is supported by the Frontier Technologies R\&D Program of Jiangsu (BF2024059), National Natural Science Foundation of China (Grants \#62025202), and the Collaborative Innovation Center of Novel Software Technology and Industrialization.
T. Chen is partially supported by overseas grants from the State Key Laboratory of Novel Software Technology, Nanjing University (KFKT2023A04,  KFKT2025A05).
Yuan Yao is the corresponding author.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section*{Reproducibility Statement}

% To facilitate the reproducibility of our work, we have made our source code available online through a public repository. All experimental details, including dataset partitions, hyperparameter configurations, and model details, are fully documented in Appendix~\ref{A:hyperparameter}. We are confident that these materials provide the necessary information to replicate our findings.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \section*{Usage of LLMs}
% Large Language Models (LLMs) were utilized exclusively as writing assistants to enhance the linguistic quality of this manuscript, focusing on improving clarity, grammar, and readability. 
% Their involvement was strictly limited to this editorial function. 
% LLMs played no role in any substantive research components, including conceptualization, experimental design, data analysis, interpretation of results, or scientific content creation. 
% All intellectual contributions, methodological developments, findings, and conclusions originate solely from the authors.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> iclr2026-3/bin.tex <==
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motivation of our work}\label{Sec:motivation}
\tl{to decide which goes to intro, which stays here}

 we can describe the 
each sample group $\mathcal{G}$ is defined as 
we consider a set-valued random variable $\mathcal{G}_\mathbf{H}$ parameterized by the random vector $\mathbf{H} = [H_1, \dots, H_N]$ each component of which is a random indicator variable. % s $\{H_i\}_{i=1}^N$, i.e.,
For a realization of $\mathbf{h}=[h_1, \cdots, h_n]$ of $\mathbf{H}$, 
%
\begin{equation}\label{Eq:group}
\mathcal{G}_\mathbf{h} := \{ X_i : i \in [N], h_i = 1 \},
\end{equation}
$\mathbf{H} = [H_1, \dots, H_N]$ satisfies that its components are independent of each other under the condition of all given features $\{X_i\}_{i=1}^N$. 

Let  $\mathcal{X}=\{X_1, \cdots, X_N\}$ be the set of all features. \tl{I am actually quite confused here, $X_i$ is normally used for the calibration set.}

\hide{
We consider a set-valued random variable $\mathcal{G}_{[S_1, \cdots, S_N]}$ where $S_i$'s are $\{0,1\}$-valued i.i.d. random variables. We have $X_i\in \mathcal{G}_{[S_1, \cdots, S_N]}$ iff $S_i=1$ for each $i\in [N]$. 

$S_i\mid Z_i$ is governed by a Bernoulli distribution where $Z_i=f(X_i)$, where $f$ denotes ... 

\[
\mathbb{P}[Y_{N+1} \in \hat{C}(X_{N+1}) \mid H_{N+1}=1] \geq 1 - \alpha
\]

We consider a set-valued random variable $\mathcal{G}_\mathbf{H}$ parameterized by the random vector $\mathbf{H} = [H_1, \dots, H_N]$ where $H_i$'s are iid, each of which is governed by a Bernoulli distribution. 
% %For a realization of $\mathbf{h}=[h_1, \cdots, h_n]$ of $\mathbf{H}$, 
% %
$\mathcal{G}_\mathbf{H}= X\subseteq \mathcal{X}$ such that $X_i\in \mathcal{G}_\mathbf{H}$ iff $H_i=1$ for all $i\in [N]$. 
}
\tl{I am not sure this is what we want. Basically, for X1,... XN, we first get Z1, ..., ZN, then we can sample a 0-1 vector to form $\mathcal{G}$ which is a set. But the event that $ X_{N+1}\in \mathcal{G}_{[S_1,\cdots, S_N]}$ looks very weird, and is not quite consistent with th previous work.}

\tl{I actually suspect here $X_i$'s do not refer to calibration set, but refer to attributes.}
 
The distribution of $\mathcal{G}_\mathbf{H}$ conditioned on $X_i$'s is given by 

\begin{equation}\label{Eq:H}
\mathbf{H} \mid \{X_i\}_{i=1}^N \sim \prod_{i=1}^N \operatorname{Bernoulli}(\mathbf{P}(S_i=1 \mid Z_i)),
\end{equation}

However, various groups $\mathcal{G}$ usually suffer from different degrees of algorithmic bias, and the groups that need to be protected (characterized by the poor conditional coverage) are typically unknown in real-world applications. \tl{examples?}

To solve this concern, existing work AFCP~\citep{zhou2024conformal} proposes 
% employ a linear decision stump 
to mine the groups that are discriminated against via the feature selection using a linear decision stump.  
% \tl{what is the formal meaning of this linear decision stump?}.
Specifically, for a test point $X_{N+1}$, they compute a conditional miscoverage score for each single \emph{discrete} feature of $X_{N+1}$ and pick the top-$k$ features with the highest scores as the selected features, where $k$ is a hyperparameter which decides the number of selected features. 
Arbitrary $X\in \mathcal{X}$ with the same value on the selected features as $X_{N+1}$ is assigned to the group $\mathcal{G}$ \tl{I do not quite understand this (unfinished?) senstence}

\tl{check this please}
Suppose there are two features: a continuous feature \textit{Age}
% \textit{Age $:=\{$Underage: 0, Adult: 1$\}$} 
and a discrete feature \textit{Gender $:=\{$Male, Female$\}$}, and $X_{N+1}$ is an instance of Male of age 50. Then one group (for Age) includes all samples with an age 50, and another group (for Gender) includes all samples who are Male. AFCP computes conditional miscoverage scores for these two groups. 




% For a decision-making process driven by machine learning (e.g., medical diagnostics, job screening and recidivism prediction) %, loan approval, fraud detection), 
% it is essential for the predictions to be accompanied by a level of confidence to quantify uncertainty~\cite{vovk2005algorithmic,smith2024uncertainty}.
% Conformal prediction (CP) is a promising uncertainty quantification method, providing statistically rigorous uncertainty sets for black-box machine learning models~\cite{babbar2022utility,straitouri2023improving,straitouri2023designing,cresswell2024conformal}. 
% %Conformal prediction (CP) is a machine learning framework for uncertainty quantification used in decision-making processes (e.g., loan approval, fraud detection)~\cite{vovk2005algorithmic,smith2024uncertainty}.  
% In standard classification, for any test input $x$, the posterior distribution $\tilde{\pi}_y(x)= P(Y=y\mid X=x)$ on classes $[K]:=\{1, \cdots, K\}$ is calculated. %This does not guarantee safe deployment. 
% Conformal prediction leverages an additional
% calibration step to guarantee a user-specified (marginal) coverage: by producing a prediction set $\mathcal{C}(x)\subseteq [K]$, it guarantees the true class of $x$ is included in $\mathcal{C}(x)$ with a user-chosen probability, % $1-\alpha$, 
% when the calibration samples are exchangeable with the test samples. 


%%%%%%%%%%%%%%%%%%%% this is just for later use %%%%%%%%%%%%%%%%
In conformal prediction, it is important to distinguish between marginal and conditional coverage guarantees. Marginal coverage ensures that, averaged over the entire data distribution, the prediction set contains the true label with probability at least 
$1-\alpha$. Formally,
$ P(Y\in \hat{C}(X))\geq 1-\alpha$,
where the probability is taken over both inputs and outputs. This guarantee is relatively easy to achieve and is what standard conformal methods provide.

By contrast, conditional coverage requires the guarantee to hold for each input (or subgroup of inputs), i.e.,
$\forall x$, $P(Y\in \hat{C}(X)\mid X=x)\geq 1-\alpha$.
This is a much stronger notion of validity, as it demands correct coverage across all regions of the feature space, not just on average. However, achieving conditional coverage is generally infeasible in finite-sample settings without making strong distributional assumptions, and attempts to enforce it often lead to excessively conservative prediction sets.

%%%%%%%%%%%%%%%%%%%%%%%%
% intuition of adaptability
% A key design consideration for conformal prediction is adaptivity: we want the procedure to return larger sets for harder inputs and smaller sets for easier inputs. 

% It is important to keep in mind that the CP procedure with the smallest average set size is not necessarily the best. A good CP procedure will give small sets on easy inputs and large sets on hard inputs in a way that faithfully reflects the model's uncertainty. This adaptavity is not implied by the marginal coverage, but it is non-negotiable in practical deployments of conformal prediction. 

% % Precise metrics for adaptivity that allow users to check a conformal procedure and to compare multiple alternative conformal procedures. 
% Adaptivity is typically formalized by the conditional coverage. That is, for each value of the input $X_{\rm test}$, we seek to return prediction sets with $1-\alpha$ coverage. This is a stronger property than the marginal coverage that CP is guaranteed to achieve. Indeed, in the most general case, conditional coverage is impossible to achieve \cite{Vovk12}, i.e., conformal procedures are not guaranteed to satisfy conditional coverage. It is imperative to check how close a CP comes to approximate it. (feature-stratified coverage metric, size-stratified coverage metric)



\textbf{Group-balanced conformal prediction}: want prediction intervals that have equal error rates across certain subsets of the data. 

Class-conditional CP

\tl{copied from Romano's paper.}
We propose a concrete procedure, which acts as a wrapper around the predictive model, to produce
perfectly valid prediction intervals that provably satisfy the equalized coverage constraint for any black box algorithm, sample size and distribution. Such a procedure can be formulated by refining tools from conformal inference, a general methodology for constructing prediction intervals [18–24]. Our contribution is nevertheless a little outside of classical conformal inference as we seek a form of conditional rather than marginal coverage guarantee [25–27].

\tl{to be adapted}
Conformal inference with \emph{equalized coverage}~\cite{romano2020malice} 
an appealing approach.

Equalized coverage aims to ensure that the prediction sets attain their coverage not only on average for the whole population (e.g., above 90\%) but also at the same level within each group of interest. While this does not necessarily imply that the prediction sets will have equal size on average across different groups, 
%—since it is possible the predictive model may be more or less accurate for different groups—
it objectively communicates the possible limitations of a model. This transparency helps decision makers recognize when predictions may be less reliable for specific subgroups, allowing them to either avoid unnecessary actions or adopt more cautious strategies in cases of higher uncertainty, thereby minimizing the potential harm from inaccurate predictions.

A limitation of %the method developed in [17] for conformal inference with 
equalized coverage is that it does not scale well to situations involving diverse populations with multiple sensitive attributes. In such cases, it necessitates splitting the data into exponentially many subsets, significantly reducing the effective sample size and leading to less informative predictions. 

Balancing this trade-off between efficiency (i.e., %aiming for 
highly informative predictions with small set sizes) and fairness (i.e.,
ensuring unbiased treatment) is challenging. % and requires novel approaches. This paper introduces
% a method to address this by providing equalized coverage conditional on carefully chosen features,
% informed by the model and data. 

While it cannot guarantee equalized coverage for all sensitive groups, it seeks a reasonable compromise with finite data sets, mitigating significant biases while
retaining predictive power.

\tl{to be adapted. This is just a placeholder}
% When multiple sensitive attributes are involved, the concept of equalized coverage is extended to \emph{exhaustive equalized coverage} \citep{zhou2024conformal}. However, a downside of this approach is that the calibration subsets may be too small if $M$ is large, leading to uninformative predictions for even moderate values of K. This limitation forms the starting point of our work. \tl{to be rephrased, basically a statistical barrier}

% \emph{Adaptively Fair Conformal Prediction.} In practice, for a given model and data set, different groups may not exhibit the same need for rigorous equalized coverage guarantees, as conformal predictions may be able to approximately achieve the desired coverage even without explicit constraints. Algorithmic bias typically affects only a minority of the population, so standard prediction sets with marginal coverage may approximately satisfy the marginal coverage for most groups. Adaptively Fair Conformal Prediction (AFCP) %, a new method that efficiently identifies and addresses groups suffering from algorithmic bias 
% was proposed in a data-driven
% way, adjusting their prediction sets to equalize coverage without sacrificing informativeness.

==> iclr2026-3/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026-3/tables/condition_per_efficiency_1.tex <==

\begin{table}[t]
    \caption{Increase in conditional coverage per efficiency w.s.t the total number of training and calibration data points on the synthetic data. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}. Our \name performs better than baselines.}
    \vskip -1em
    \label{T:C/E}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{sc}
    \begin{tabular}{l|cc|cc|cc|cc|cccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} & \multicolumn{2}{c|}{$N=3000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
    \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
    & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ \\ 
    \midrule
     Partial  & 0.210 & 0.209 & 0.243 & 0.252 & 0.289 & 0.287 & 0.274 & 0.258 & 0.228 & 0.231\\
     AFCP1    & \underline{0.215} & \underline{0.214} & \underline{0.262} & \underline{0.267} & 0.291 & 0.304 &  0.262   &  
     0.232    & \underline{0.261} & 0.257\\
     AFCP2    & 0.111 & 0.104 & 0.245 & 0.240 & \underline{0.334} & \underline{0.327} &  \underline{0.298}   &  
     \underline{0.278}    & 0.259 & \underline{0.301}\\
     \midrule
     \name    & \textbf{0.219} & \textbf{0.217} & \textbf{0.311} & \textbf{0.296} & \textbf{0.390} & \textbf{0.381} &  \textbf{0.378}   &  \textbf{0.325}    & \textbf{0.337} & \textbf{0.314} \\
    \bottomrule
    \end{tabular}
    \end{sc}}
    \end{center}
\end{table}



% \begin{table}[t]
%     \caption{The accuracy of two different models on the four math reasoning datasets. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}.}
%     \vskip -1em
%     \label{tab:model-and-scales}
%     \begin{center}
%     \resizebox{\textwidth}{!}{
%     \begin{sc}
%     \begin{tabular}{l|cc|cc|cc|cc|cccc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=200$} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
%     \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
%     & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ \\ 
%     \midrule
%      Partial & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx\\
%      AFCP1 & 0.148 & 0.165 & 0.215 & 0.250 & 0.262 & 0.258 & 0.291 & 0.317 & 0.261 & 0.336\\
%      AFCP2 & 0.053 & 0.065 & 0.111 & 0.114 & 0.245 & 0.248 & 0.334 & 0.347 & 0.259 & 0.331\\
%      \midrule
%      \name & 0.150 & 0.167 & 0.219 & 0.251 & 0.311 & 0.312 & 0.390 & 0.420 & 0.337 & 0.353\\
%     \bottomrule
%     \end{tabular}
%     \end{sc}}
%     \end{center}
% \end{table}

==> iclr2026-3/tables/condition_per_efficiency_2.tex <==

\begin{table}[t]
    \caption{Increase in conditional coverage per efficiency w.s.t the total number of training and calibration data points on the nursery data. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}. Our \name performs better than baselines.}
    \vskip -1em
    \label{T:C/E}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{sc}
    \begin{tabular}{l|cc|cc|cc|cc|cccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} & \multicolumn{2}{c|}{$N=3000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
    \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
    & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ \\ 
    \midrule
     Partial  & 0.210 & 0.209 & 0.243 & 0.252 & 0.289 & 0.287 & 0.274 & 0.258 & 0.228 & 0.231\\
     AFCP1    & \underline{0.215} & \underline{0.214} & \underline{0.262} & \underline{0.267} & 0.291 & 0.304 &  0.262   &  
     0.232    & \underline{0.261} & 0.257\\
     AFCP2    & 0.111 & 0.104 & 0.245 & 0.240 & \underline{0.334} & \underline{0.327} &  \underline{0.298}   &  
     \underline{0.278}    & 0.259 & \underline{0.301}\\
     \midrule
     \name    & \textbf{0.219} & \textbf{0.217} & \textbf{0.311} & \textbf{0.296} & \textbf{0.390} & \textbf{0.381} &  \textbf{0.378}   &  \textbf{0.325}    & \textbf{0.337} & \textbf{0.314} \\
    \bottomrule
    \end{tabular}
    \end{sc}}
    \end{center}
\end{table}





==> iclr2026-3/tables/hyperparameter.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{Hyperparameters of \name.   \label{T: hyperparameters}}
%     \resizebox{\linewidth}{!}{
%     \begin{sc}
%     \begin{threeparttable}
%       \begin{tabular}{lcccccccc}
%        \toprule
%         {Dataset} & Model & Number of Layers & Hidden dimension & Epoch & Learning Rate & $\beta$ & $\delta$ & $T$  \\
%         \midrule
%         {Synthetic Data} & MLP & 3 & [64,32] & 2000 & 0.001 & 2 & 0.3 & 10\\
%         {Nursery Data} & MLP & 3 & [64,32] & 800 & 0.01 & 0.1 & 0.1 & 100\\
%       \bottomrule
%       \end{tabular}
%     \end{threeparttable}
%     \end{sc}
%     }
 
% \end{table*}


\begin{table*}[h]
    \centering
    \caption{Hyperparameters of \name.   \label{T:hyperparameters}}
    \resizebox{0.7\linewidth}{!}{
    \begin{sc}
    \begin{threeparttable}
      \begin{tabular}{lcc}
       \toprule
        {Dataset} & Synthetic Data & Nursery Data   \\
        \midrule
        {Model} & MLP & MLP \\
        {Number of Layers}& 3 & 3 \\
        {Hidden dimension}& [64,32] & [64,32] \\
        {Epoch}& 2000 & 800 \\
        {Batch Size}& 500 & 500 \\
        {Learning Rate}& 0.001 & 0.01 \\
        {$\beta$}& 2.0 & 0.1 \\
        {$\delta$}& 0.3 & 0.1 \\
        {$T$}& 20 & 100 \\
      \bottomrule
      \end{tabular}
    \end{threeparttable}
    \end{sc}
 }
\end{table*}

==> iclr2026-3/tables/time.tex <==
\begin{table*}[t]
    \centering
    \caption{Time cost.}
    \label{T:time}
    \vskip 0.05in
    \resizebox{0.4\linewidth}{!}{
      \begin{sc}
      \begin{tabular}{lccc}
      \toprule
      {N} & AFCP1 & AFCP2 & Ours\\
      \midrule
      % 200 & 213.06 & 208.27 & 25.10\\
      500 & 529.04 & 528.29 & 36.68\\
      1000 & 1080.43 & 1080.01 & 59.33\\
      2000 & 2349.87 & 2347.20 & 118.25\\
      3000 & 3681.29 & 3685.10 & 183.66\\
      4000 & 4016.89 & 4017.39 & 241.42\\
      % \midrule
      \bottomrule
      \end{tabular}
      \end{sc}
      }
\end{table*}

==> tables/condition_per_efficiency_1.tex <==

\begin{table}[t]
    \caption{Increase in conditional coverage per efficiency w.s.t the total number of training and calibration data points on the synthetic data. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}. Our \name performs better than baselines.}
    \vskip -1em
    \label{T:C/E}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{sc}
    \begin{tabular}{l|cc|cc|cc|cc|cccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} & \multicolumn{2}{c|}{$N=3000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
    \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
    & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ \\ 
    \midrule
     Partial  & 0.210 & 0.209 & 0.243 & 0.252 & 0.289 & 0.287 & 0.274 & 0.258 & 0.228 & 0.231\\
     AFCP1    & \underline{0.215} & \underline{0.214} & \underline{0.262} & \underline{0.267} & 0.291 & 0.304 &  0.262   &  
     0.232    & \underline{0.261} & 0.257\\
     AFCP2    & 0.111 & 0.104 & 0.245 & 0.240 & \underline{0.334} & \underline{0.327} &  \underline{0.298}   &  
     \underline{0.278}    & 0.259 & \underline{0.301}\\
     \midrule
     \name    & \textbf{0.219} & \textbf{0.217} & \textbf{0.311} & \textbf{0.296} & \textbf{0.390} & \textbf{0.381} &  \textbf{0.378}   &  \textbf{0.325}    & \textbf{0.337} & \textbf{0.314} \\
    \bottomrule
    \end{tabular}
    \end{sc}}
    \end{center}
\end{table}



% \begin{table}[t]
%     \caption{The accuracy of two different models on the four math reasoning datasets. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}.}
%     \vskip -1em
%     \label{tab:model-and-scales}
%     \begin{center}
%     \resizebox{\textwidth}{!}{
%     \begin{sc}
%     \begin{tabular}{l|cc|cc|cc|cc|cccc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=200$} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
%     \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
%     & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ & $\Delta C/\Delta E$ & $\Delta W/\Delta E$ \\ 
%     \midrule
%      Partial & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx\\
%      AFCP1 & 0.148 & 0.165 & 0.215 & 0.250 & 0.262 & 0.258 & 0.291 & 0.317 & 0.261 & 0.336\\
%      AFCP2 & 0.053 & 0.065 & 0.111 & 0.114 & 0.245 & 0.248 & 0.334 & 0.347 & 0.259 & 0.331\\
%      \midrule
%      \name & 0.150 & 0.167 & 0.219 & 0.251 & 0.311 & 0.312 & 0.390 & 0.420 & 0.337 & 0.353\\
%     \bottomrule
%     \end{tabular}
%     \end{sc}}
%     \end{center}
% \end{table}

==> tables/condition_per_efficiency_2.tex <==

\begin{table}[t]
    \caption{Increase in conditional coverage per efficiency w.s.t the total number of training and calibration data points on the nursery data. The best performance is highlighted in \textbf{bold}, while the second-best performance is \underline{underlined}. Our \name performs better than baselines.}
    \vskip -1em
    \label{T:C/E}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{sc}
    \begin{tabular}{l|cc|cc|cc|cc|cccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$N=500$} & \multicolumn{2}{c|}{$N=1000$} & \multicolumn{2}{c|}{$N=2000$} & \multicolumn{2}{c|}{$N=3000$} &  \multicolumn{2}{c}{$N=4000$}\\ 
    \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \cmidrule{10-11} 
    & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ & $\Delta G/\Delta E$ & $\Delta W/\Delta E$ \\ 
    \midrule
     Partial  & 0.210 & 0.209 & 0.243 & 0.252 & 0.289 & 0.287 & 0.274 & 0.258 & 0.228 & 0.231\\
     AFCP1    & \underline{0.215} & \underline{0.214} & \underline{0.262} & \underline{0.267} & 0.291 & 0.304 &  0.262   &  
     0.232    & \underline{0.261} & 0.257\\
     AFCP2    & 0.111 & 0.104 & 0.245 & 0.240 & \underline{0.334} & \underline{0.327} &  \underline{0.298}   &  
     \underline{0.278}    & 0.259 & \underline{0.301}\\
     \midrule
     \name    & \textbf{0.219} & \textbf{0.217} & \textbf{0.311} & \textbf{0.296} & \textbf{0.390} & \textbf{0.381} &  \textbf{0.378}   &  \textbf{0.325}    & \textbf{0.337} & \textbf{0.314} \\
    \bottomrule
    \end{tabular}
    \end{sc}}
    \end{center}
\end{table}





==> tables/time.tex <==
\begin{table*}[t]
    \centering
    \caption{Time cost.}
    \label{T:time}
    \vskip 0.05in
    \resizebox{0.4\linewidth}{!}{
      \begin{sc}
      \begin{tabular}{lccc}
      \toprule
      {N} & AFCP1 & AFCP2 & Ours\\
      \midrule
      % 200 & 213.06 & 208.27 & 25.10\\
      500 & 529.04 & 528.29 & 36.68\\
      1000 & 1080.43 & 1080.01 & 59.33\\
      2000 & 2349.87 & 2347.20 & 118.25\\
      3000 & 3681.29 & 3685.10 & 183.66\\
      4000 & 4016.89 & 4017.39 & 241.42\\
      % \midrule
      \bottomrule
      \end{tabular}
      \end{sc}
      }
\end{table*}
